DramaChain Bench: An End-to-End Benchmark for Short-Drama Generation

Commercial short-drama production follows a multi-stage chain: script, storyboard, keyframe imagery, shot-level video, and the finished short drama. Most existing benchmarks evaluate solely the video-generation stage using pre-authored inputs instead of real upstream pipeline outputs. This leaves two critical questions unanswerable: whether each stage adheres to the original script intent (rather than only its immediate input prompt), and whether disparate shots remain coherent after assembly into multi-episode releases. We present DramaChain Bench, the first short-drama benchmark that evaluates every stage of the complete production chain. It is built upon three in-house systems sharing one dimension system, DramaChain Dimensions: five evaluation axes instantiated at every stage, resolving into 63 leaf dimensions. DramaChain Agent is calibrated against commercial short-drama platforms in both workflow and finished short-drama quality, enabling stage-wise fair comparison across models. DramaChain Labeling System has each of the 5,785 items scored independently by three professional annotators, with all defects spatio-temporally localised and selected from a predefined defect list. This process produces 17,488 valid scores and 255,925 traceable attribution records. The human annotations confirm that upstream defects cascade across the pipeline, demonstrating that final episode quality is not governed by video generation alone. DramaChain Agentic Judge then scores every leaf dimension automatically, gathering evidence over multiple agentic rounds before judging against a per-item checklist; it reproduces the model ranking at a mean PLCC of 0.918, enough to admit new models at no annotation cost.

==> preamble_zh.tex <==
% ---------------------------------------------------------------------------
%  Chinese companion preamble.  Requires XeLaTeX.
%
%  This file loads the shared English preamble unchanged, then adds CJK
%  typesetting and flips the \zhen switch so that shared figures and tables
%  render their Chinese caption instead of the English one.
%
%  Everything in figures/ is shared between the two versions: only the
%  captions are bilingual, the axis labels and node text inside the plots
%  stay English so that a change to a figure never has to be made twice.
% ---------------------------------------------------------------------------

\input{preamble}

% xeCJK and the Fandol fonts are loaded by preamble.tex, which both roots share.

% Chinese text is denser than English; loosen the leading a little.
\linespread{1.16}\selectfont

% Localise LaTeX's generated strings.
\renewcommand{\abstractname}{摘要}
\renewcommand{\contentsname}{目录}
\renewcommand{\refname}{参考文献}
\renewcommand{\bibname}{参考文献}
\renewcommand{\appendixname}{附录}
\renewcommand{\figurename}{图}
\renewcommand{\tablename}{表}

% Flip the bilingual switch: take the Chinese argument.
\renewcommand{\zhen}[2]{#2}

% Chinese convention: no paragraph indent, small vertical gap instead.
\setlength{\parindent}{0pt}
\setlength{\parskip}{0.55em plus 0.1em minus 0.1em}

% cleveref in Chinese.  Sections read "4.1 节", not "第 4.1", which is what a
% straight name substitution would give.
\crefformat{section}{#2#1#3 节}
\Crefformat{section}{#2#1#3 节}
\crefrangeformat{section}{#3#1#4--#5#2#6 节}
\crefmultiformat{section}{#2#1#3 节}{ 与 #2#1#3 节}{、#2#1#3 节}{ 与 #2#1#3 节}
\crefformat{subsection}{#2#1#3 节}
\Crefformat{subsection}{#2#1#3 节}
\crefmultiformat{subsection}{#2#1#3 节}{ 与 #2#1#3 节}{、#2#1#3 节}{ 与 #2#1#3 节}
\crefformat{subsubsection}{#2#1#3 节}
\Crefformat{subsubsection}{#2#1#3 节}
\crefname{table}{表}{表}
\Crefname{table}{表}{表}
\crefname{figure}{图}{图}
\Crefname{figure}{图}{图}
\crefname{subfigure}{图}{图}
\crefname{appendix}{附录}{附录}
\Crefname{appendix}{附录}{附录}
\crefname{equation}{式}{式}
\Crefname{equation}{式}{式}


==> sections_zh/00_abstract.tex <==
\begin{abstract}
\noindent
短剧的商业化生产遵循一条多环节链路：剧本、分镜脚本、分镜图、分镜视频，以及最终的多集成片。
现有基准大多只评测其中的视频生成一环，且使用人工构造的题面，而非产线上游的真实产出。
这使两个关键问题无法回答：各环节是否忠实于原始\emph{剧本}意图（而不只是它这一环的输入提示词），
以及各个独立生成的镜头在剪成多集成片之后是否仍然彼此协调。
本文提出 \bench{}，首个对完整生产链路每一环都评测的短剧基准。它建立在三套自研系统之上，
三者共用同一套维度体系 \dimsys{}：五条评测轴在每个环节上各自实例化，细化为 $63$ 个叶子维度。
\pipe{} 在生产流程与成片质量两方面对标商用短剧平台，使各环节的模型比较公平可比。
\labeler{} 为参考集中 $5{,}569$ 道题的每一道提供三份独立的专业评分，缺陷在适用时进行时空定位，
并从预设的缺陷词表中选取；
全部标注采集共产出 $17{,}488$ 份有效打分与 $255{,}925$ 条可追溯的归因记录。
受控替换实验显示上游缺陷会沿链路传递，最终成片质量并不只由视频生成一环决定。
\judger{} 随后自动为每个叶子维度打分：先迭代调用工具取证，再依据逐题核查清单出分；
它与人工评分的模型级 PLCC 平均达到 $0.918$。
基于这一框架，我们评测了 $37$ 个生成模型（$20$ 个文本大模型、$8$ 个图像模型、$9$ 个视频模型），其中 $22$ 个有人工标注。
在这些标注上经监督微调与 GRPO 训练的判分模型，与人工评分的一致性高于提示式的 agentic 判分系统。
\end{abstract}


==> sections_zh/01_intro.tex <==
\section{引言}
\label{sec:intro}

短剧已经成为生成式视频最重要的落地场景之一。
$2025$ 年全球微短剧收入达到 $110$ 亿美元，$2026$ 年预计为 $140$ 亿美元。
中国贡献了 $2025$ 年收入的约 $83\%$，海外市场增长很快，
Omdia 预计 $2026$ 年中国以外市场收入为 $30$ 亿美元~\citep{omdia2025,omdia2026}。
商业平台已经形成一套成熟通用的生产范式。OiiOii、Flova、小云雀、LibTV 接收用户给出的故事设定，
执行分阶段流水线：撰写剧本、拆解成分镜、渲染关键帧图像、
将关键帧动画化为分镜视频，最终剪辑合成多集成片。
学术研究也走向了同样的范式，尤以智能 Agent 框架最为典型：
Agent 流水线将每个环节分配给专门角色，上一环节产出交付给下一环节继续处理~\citep{vimax,mavis,animaker}。
由此可见，工业平台与学术论文构建的是同一套体系：一条链式流水线，每个环节消费上游输出，
因此前序环节交付给下游的结果，决定了后续所有环节能力的上限。

尽管生产链路已经成熟，但评测体系并没有跟上这条流水线的思路。
第一代评测基准针对单条视频片段，基于模型层面的人类偏好对各项能力维度打分~\citep{vbench,vbench2}；
第二代以 FilmBench~\citep{filmbench} 为代表，将评测对象拓展到电影语言与多镜头场景~\citep{msvbench,entitybench,vistorybench}；
第三代开始按照生产流水线组织评测指标~\citep{evalverse,directorbench}。
但它们都不评估流水线上一个环节交付给下一环节的那份产物。
即使在短剧域内的基准中给这类中间产物打了分，那份产物也是从已完成的短剧中挖出来的，
而不是被测流水线自己产出的~\citep{dramadirector}。
由此有三点局限。
（1）\textbf{各环节都是被隔离开单独测的}，
因此无法判定成片缺陷来自哪一环，也无法量化它向下游传了多远。
（2）\textbf{题面是为评测而撰写的，而不是流水线产出的}（反向构造的提示词、从已有素材里截的镜头），
因此它干净且自足，不同于产线上一环真正收到的那份机器产物。
（3）\textbf{监督信号无法定位缺陷}：人工标注以模型级相关性校验指标，
即使逐题标注，记下的也是偏好或整体印象分，而不是哪个维度出错、错在哪里、为何出错，
于是打分器只能被验证排名对不对，无法被验证是否找到了缺陷。

针对这三点，我们提出 \bench{}：一个对完整生产链路每一环都打分的短剧基准，
且题面由这条链路自己产出。
五条评测轴（输入保真、内部一致、生成合理、视觉质量、影视表现力）只定义一次，
再在六个粒度上实例化，细化为 $63$ 个叶子维度；参考集包含 $5{,}569$ 道有完整三人标注的题。
为解决前文提到的这些问题，\bench{} 依托我们自研的三套系统构建（\cref{fig:overview}）。

\input{figures/fig_overview}

\pipe{} 以全自动方式端到端执行一条完整的短剧生产链路：
基于给定剧本，为构成本基准基础的 $20$ 部短剧、共 $60$ 集生成分镜、分镜图、分镜视频与成片。
它的工作流程与输出的短剧质量都对标真实生产平台，
这样的设计使被评的对象不会变成一条有缺陷的产线本身。
该框架只在被测环节处分叉：参评模型获得完全相同的上游产物与提示词，其余环节保持固定。
\labeler{} 由三名专业标注员在全部适用维度上对每道题独立打分，
每个叶子维度都配一套五档可判定判据；各档定义可观察的判定条件，
并映射到一套封闭的归因标签词表，扣分在适用时进行时空定位。
由此得到 $543$ 名标注员贡献的 $17{,}488$ 份打分与 $255{,}925$ 条可复核归因。
\judger{} 自动复现这份人工参照：它汇总按各维度判据路由而来的度量，
并可迭代调用外部工具，最终依据逐题核查清单给出判定，
与人工标注面板的模型级 PLCC 平均达到 $0.918$。

本文对 $22$ 个模型做了人工标注评测（$9$ 个文本 LLM、$7$ 个图像模型、$6$ 个视频模型），
覆盖各模型实际产出的每道题与每个适用维度（覆盖缺口见 \cref{sec:cov}）；另有 $15$ 个仅由 \judger{} 打分、没有人工标注的模型。
按自动化评分，可交付的配置存在：在有人工标注的模型中，\md{gpt-5.5-xhigh}、\md{gpt-image-2}、\md{seedance-2.0}
各自领跑所在环节，串联得到的成片 $3.30$ 分，在 $3.0$ 可用线以上；\md{seedance-2.5} 的成片达到 $3.70$ 分。
而上游环节的缺陷会沿链路累积传导、不会留在原地（按受控替换实验的自动化评分，只降级一个上游环节，
单条片段付出 $0.07$--$0.13$ 分，而交付的成片付出 $0.25$--$0.83$ 分），
因此最终成片质量并不只由视频生成一环决定。
自动化评测与这张榜的模型级 PLCC 平均为 $0.918$，
而在标注数据上训练的判分模型与人工评分的一致性还高于提示式判分系统（\cref{sec:judgetrain,sec:ablation}）。

\bench{} 支持可扩展的评测，而不是一次性的静态基准：
环节级分叉机制让新模型只需完成单个环节的生成即可接入，自动化评测则减少了将其放上榜单所需的人工标注。
我们将开放全部基准数据、判分模型以及 \pipe{} 生成流水线。


==> sections_zh/02_related.tex <==
\section{相关工作}
\label{sec:related}

\subsection{叙事视频生成}
\label{sec:rw:gen}

一条路线在单个模型内部产出整段多镜头叙事，而不搭分环节流水线：HoloCine~\citep{holocine}
以稀疏跨镜头注意力对整场戏联合去噪，CausalCine~\citep{causalcine} 以自回归方式跨镜头边界实时生成。
其余工作大多在做记忆：持续更新的关键帧库、按实体索引的记忆库、
在镜头边界上门控的记忆槽、带自适应遗忘的场景回忆，
以及逐段对照多模态记忆反复自我修正的闭环~\citep{storymem,emvid,unityshots,echoforcing,videomemory,a2rd}；
另有一篇把问题放到别处：ReCA~\citep{reca} 放在上下文\emph{如何分配}而不是有多长。
控制则通过相机路径、关键帧条件或分镜草图暴露~\citep{shotdirector,smartdirector,drawvideo}。
记忆这一支文献如此之大，本身就是结论：长程一致性随距离衰减。
而控制粒度仍然粗：一句提示词、一条相机路径或一张草图都不是逐环节的规格说明，
因此某条要求做错了，无法只把它重新下发给负责的那一环，只能整段重新生成。

第二条路线把问题分解为彼此传递产物的分环节角色，各家的差别主要在环节切在哪里、以及是否在产出之上再加搜索。
最早的一批是动画系统：Anim-Director~\citep{animdirector} 由一个大型多模态模型驱动一条可控的动画链路，
AniMaker~\citep{animaker} 承其后，改为多智能体生成，并以蒙特卡洛树搜索的思路搜索候选片段。
UniVA~\citep{univa} 把同一思路带到任意视频任务上，做成工具服务器之上的规划与执行智能体；
MAViS~\citep{mavis} 与 ViMax~\citep{vimax} 则搭起完整的叙事链路，
把剧本、镜头设计、角色造型、关键帧与动画分派给各自专职的智能体，其中 MAViS 还覆盖音频；
Co-Director~\citep{codirector} 用多臂老虎机搜索创意方向，
Soap2Soap~\citep{soap2soap} 把同样的分工用于整部剧的重制。
其中有两个系统面向短剧：DramaDirector~\citep{dramadirector} 把规划锚定在从真实短剧镜头中检索出的几何上；
One Sentence One Drama~\citep{onedrama} 用多智能体辩论约束节奏并做分阶段复核，
以此把剧本生成与制作耦合起来；
两者都把难点定位在环节的交接上：文本分镜脚本给不出渲染所需的几何，
而剧本、帧图与视频各环节累积的误差，若无复核回路就不会被纠正。
商用平台跑的也是同一形态的框架（\cref{sec:intro}），
这正是逐环节评测既成为可能、也成为必要的原因，也是本基准所站的位置。

\subsection{数据集与基准}
\label{sec:rw:bench}

已有语料为这些系统提供了素材，但不是一个链路级基准所需要的东西。
它们都是从被测产线之外的素材中大规模汇集而来：电影级素材、多镜头语料、
从真人短剧里挖出的镜头，以及以网络视频为底、部分参考图由模型合成的主体一致三元组~\citep{moviebench,%
muss,cinedance,dramadirector,opens2v}。
其中始终缺两样东西。
一是没有一份语料记录\emph{完整的生成链路}（同一集的剧本、分镜脚本、分镜图、分镜视频与成片，
由同一条产线产出），因此任何一环的输入都是人做出来的产物，
而不是真实部署里会喂给这一环的那个模型的输出。
二是没有一份语料带有\emph{定位}并\emph{归因}错误的标注：
标注是整条片段级的评分或字幕，所以语料能确立「这条比那条差」，
却不记录缺陷在哪里、由什么造成，而这恰恰是把缺陷记到某一环上所必需的信号。

基准的发展经历了三步。
VBench~\citep{vbench,vbench2} 确立了模板：把质量拆成若干能力维度，
每个维度用通用 VLM 或专用检测器实现，再用模型级的人类偏好校验整套。
第一批工作在此之上细化，转向基于 MLLM 的打分、补上逐样本归因、
试探全模态大模型作为评判者能被信任到什么程度、
以及把物理常识单独隔出来考察~\citep{videobench,videogeneval,qsave,omnijudge,videophy2}；
反复出现的结论是这类评判者在语义对齐上有竞争力、在任何需要高时间分辨率的地方都弱，
本报告在维度层面复现了同一分野（\cref{sec:meta}）。
第二波工作保留这一模板而延伸评测目标（影视语言、跨镜一致、分镜面板、
多人对话与多参考的有声视频、叙事丰富度、长组合提示词、记忆，以及分钟级生成~\citep{filmbench,msvbench,%
entitybench,vistorybench,mtavg2,multiref,narrlv,locot2v,vgifscore,mbench,longav}），
另有一支专门考察视觉语言模型是否读得懂摄影语言~\citep{cinetech,shotbench}；
但被打分的始终是一件成品产物，而不是产出它的那些交接。
VideoWeaver~\citep{videoweaver} 正好划出这条边界：它的判分者确实会读 agent 的执行轨迹与中间文件，
但问的是工作流有没有把步骤跑完，而不是每件中间产物是否达到某条评分标准。
同一趋势在视频之外也能看到：在文生图上，
Qwen-Image-Bench~\citep{qwenimagebench} 用与职业创作者共同设计的可核查评分细则，
取代了提示词层面的对齐分。
最接近的工作把评测与工作流本身对齐：
EvalVerse~\citep{evalverse} 是「管线感知」的，但与工作流对齐的是\emph{判据}，
题面仍然作为成品视频被评价，因此缺陷无法记到某一环上；
DirectorBench~\citep{directorbench} 记录每个检查点是否通过，
并把瓶颈定位在单元之间而不是单元之内，这与本报告在 \cref{sec:prop} 得到的结论形状相同，
但它从不依据判据给一个环节交给下一环节的产物打分。
在短剧领域内，评测集都附属于某个生成系统，且仍未走到整条链路：
评剧本续写、在真实短剧挖出的分镜上评分镜与视频，或把整条链路当黑盒~\citep{dramabenchscript,%
dramadirector,onedrama}。
\cref{tab:related} 给出 \bench{} 与上述文献的对照，其中有两条性质在此前的每一行上都成立：
题面或为评测而撰写、或从已有成片中剪出，
因此被测环节的输入从来不是那个真正会喂给它的模型产出的；
而人工标注用于以模型级相关性校验一个指标，因此即使逐题标注，
记下的也是偏好或整体印象分，而不是逐维度打分并把扣分定位下来。

\input{figures/tab_related}


==> sections_zh/03_benchmark.tex <==
\section{\bench}
\label{sec:bench}
\label{sec:benchmark}

\bench{} 交付的不是一个数据集，而是三块自建基础设施与 \dimsys{}。
\textbf{\dimsys{}}（\cref{sec:dims}）：六个环节共用同一套五条评测轴，
因此同一条判据可以沿链路一路追下去，上游缺陷对下游的影响才成为可观测量。
\textbf{\pipe{}}（\cref{sec:sourcing}）：题面是跑出来的而不是写出来的，
产线成片水平对标商用短剧平台，且只在被测环节分叉，因此模型之间逐环节可比。
\textbf{\labeler{}}（\cref{sec:annot}）：三名标注员独立打分，
每次扣分都落到时空位置并取归因标签，由此可以验证自动化判分是否找对了缺陷，而不只是给对了分数。
\textbf{\judger{}}（\cref{sec:judge}）：不让小模型指标直接喂给大模型判分，
而是先按与人工的一致性筛掉无效指标，再迭代调用 agentic 工具取证，最后依逐条核查清单出分。这份清单用的是标注员所用的同一份判据文本与缺陷词表。

\subsection{\dimsys{}：六个环节共用五条轴，细化为 $63$ 个叶子维度}
\label{sec:dims}

六个环节共用同一套五条评测轴；而共用它们，正是缺陷从「看得见」变为「追得到」的原因。
一份把多个动作塞进同一个镜头的分镜，会在 \axP{} 上因可执行性被扣分，
而由这份分镜生成的镜头会再一次在 \axP{} 上被打分；
于是一条在物理上不成立的视频，可以对照它所收到的那条指令本身是否可行来读，
而不是默认记到视频模型头上。这类缺陷能传多远，由 \cref{sec:prop} 度量。

\axF{}\textbf{输入保真}问这一环有没有按输入要求做，拿上游产物核对。
\axC{}\textbf{内部一致}问这是不是与另一镜里同一个人、同一处场景、同一件道具，拿同级产物核对。
\axP{}\textbf{生成合理}问这在物理与因果上可不可能，没有外部参照物。
\axQ{}\textbf{视觉质量}是像素的技术与美学质量，纯感知。
\axE{}\textbf{影视表现力}涵盖构图、运镜、表演、音效设计与可看性：感知加审美。
这些轴之下的每个叶子维度另配五档可判定描述与一组固定的归因标签，
且\textbf{人工与自动化评测读的是同一份判据文本，并从同一套词表中取缺陷标签}（\cref{sec:tagvocab}）。
\cref{fig:teaser} 给出由此得到的矩阵；哪条轴在哪个环节激活、逐维完整定义，
以及 schema 自身的计数口径，均见 \cref{app:dims}。

\input{figures/fig_teaser}


\subsection{\pipe{}：搭建一套对标商用平台的短剧生产系统}
\label{sec:sourcing}

题面由一条产线产出，而不是为评测而撰写。\pipe{} 是本基准所依托的短剧生成 agent 系统，
它基于 ViMax 框架~\citep{vimax} 开发，其链路自商用平台逆向而来并在此基础上做了优化。
在被评的六个环节之外，它还产出一条产线所需的中间产物：
角色立绘、场景与关键元素参考图、逐镜描述以及摄像机树。它有以下三项特点。

\input{figures/fig_sourcing}

\paragraph{多元数据。}
$20$ 部短剧 $\times$ $3$ 集连续集数 $=60$ 集，按频道、年代主题与题材铺开，
并与画风（真人 / 动画，$10$:$10$）和台词语言（中文 / 英文，$16$:$4$）交叉，
使每个切面都够做分层核查。剧本是给定的输入，而非链路产出；
每部剧有统一的角色名册，并遵循商用拍摄稿格式（\cref{app:dramas}）。
\cref{fig:corpus} 取自二十部剧中八部的八道题，完整清单见 \cref{app:dramas}。

\input{figures/fig_corpus}

\paragraph{对标商用平台。}
一条弱产线生成的基准衡量的是产线而不是模型，因此链路、驱动环节的方式与产出效果三方面都要对标。
链路就是那些平台从剧本往下跑的链路：分镜脚本、分镜图、分镜视频，直到成片，全程自动。
平台之间还有一处不同在于\emph{以何种形态}驱动视频环节，\pipe{} 实现了四种输入范式，
它们的区别在于交给视频模型的那份产物（\cref{fig:sourcing}）：首尾帧对（\texttt{fflf2v}）、
切开的宫格图（\texttt{grid2v}）、只给角色/元素/场景参考而不给帧图（\texttt{multiref2v}），
或独立绘制的多关键帧（\texttt{keyframe2v}）。本期评了前三种。
产出效果方面，我们把同一份剧本端到端跑过 \pipe{} 与三个商用短剧平台，
全自动、无人工剪辑、无挑帧、无重跑择优；经专家评测，分镜切分、角色与场景一致、
镜头语言与音轨都落在同一档，差别在各家的风格取向上。
\cref{fig:parity} 展示了四个系统在同一份剧本（三场戏、八个镜头）上的产出；它说明的是一种实际生产场景，
而不是一次受控的平台对比。\cref{fig:exhibit} 展示了 \pipe{} 产出的一部剧的三集，按等间隔抽帧，
用来说明单个镜头之外所需的连续性。

\input{figures/fig_parity}

\paragraph{逐环节可比。}
两个模型的分差必须只来自模型本身。在每个粒度上，同一镜位由每个参评模型各生成一份；
且链路只在被评环节分叉（\cref{fig:sourcing}）：分叉之前的一切只生成一次，
因此参评模型拿到的是完全相同的上游产物与同一份提示词，
而评测一个新模型只需付出一个环节的生成成本，不必重造语料。
覆盖缺口与时长预算例外逐项列在 \cref{sec:cov}。

\subsection{\labeler{}：以信息量与区分力为目标的标注}
\label{sec:annot}

同类既有工作通过小样本打分或方法级对照来构建其人工评测层，而不是逐题穷尽覆盖；
这类做法只能验证模型级的排名结果。相比之下，\labeler{} 采用专业标注人力、
逐题多维打分与强制时空归因（\cref{fig:annotation}）。
全部标注采集共得到 $17{,}488$ 条打分与 $255{,}925$ 条可验证归因，单题标注耗时中位数为 $23$ 分钟。
标注协议要求每道题由三名标注员独立打分；参考集由具备全部三份评分的 $5{,}569$ 道题构成，
上述采集总量并不限于参考集。由于扣分在适用时都被定位并赋予归因，
我们得以验证自动化打分是否识别出了真正的底层缺陷，而不只是给出了一个看似合理的最终分数。

\input{figures/fig_labeling}

\paragraph{标注人员画像。}
我们的标注池共有 $543$ 名标注员。招募采用分环节的技能筛选：
分镜设计环节的标注员须具备导演或编剧背景，其他环节的标注员则需具备丰富的图像或视频标注经验。
标注任务分发给多个供应商团队，每个团队各自运作自己的标注员队伍与专职质检人员。

\paragraph{时空归因。}
对于任何未获满分的维度，标注员必须在适用时定位问题，并从该维度预设的标签集中选择相应理由。
标注界面随任务环节动态适配，支持画框选帧、时间区间、单个或区间镜号，以及自由文本输入。
这条核心约束支撑起本文其余部分的分析：它把「三名标注员都不喜欢某个产出」
与「三名标注员指向同一处缺陷」区分开；它定义了自动化打分必须遵循的标准化输出格式；
并且它能自动暴露没有证据支撑的扣分。

\paragraph{质量控制与过滤。}
\label{sec:filter}
组级质检按可配置的比例抽检本组产出（默认五分之一）。未通过的标注存档留底并重新派发返修。
质量看板还依据九条启发式规则进一步标记低质量提交以供修订，
包括标注用时远低于同粒度中位数、扣分却无对应归因，
以及与留一共识的相关性接近于零。

\paragraph{共识与人工基线。}
人工共识在叶子维度与综合分两个层面上都取可用标注员评分的均值。
为了给自动化一致性提供参照，留一法人工基线 \hbase{} 计算每名标注员的评分与其余标注员均值之间的 PLCC，并汇总全部配对。
\judger{} 在同时具有人工与自动评分的题目上与标注员均值比较（\cref{tab:agree}）。

\subsection{\judger{}：多工具 agentic 判分}
\label{sec:judge}

\input{sections_zh/04_judge}


==> sections_zh/04_judge.tex <==
\paragraph{基线方法与混合方案。}
基线做法是把输入素材与评测判据直接喂给一个 VLM，产出单个 JSON 格式的判定。
它有一个根本性的结构缺陷：短剧的缺陷往往位于帧内的局部区域，或位于段与段之间的不连续处，
而基于整体印象的评估对两者都看不见。
已有的混合方案通过给大模型配上专家小模型的度量来缓解这一点~\citep{msvbench,entitybench,multiref}。
沿着这一范式，我们接入了完整的一套模块：检测与分割~\citep{yolo26,sam2}、
身份与通用视觉相似度取证~\citep{arcface,dinov3}、场景一致性~\citep{dreamsim}、风格一致性~\citep{csd}、
美学质量~\citep{musiq,nima,dover}、运动~\citep{raft}、
音频分析~\citep{whisper,dnsmos,syncnet,imagebind}，以及以 VideoPhy-AutoEval 做跨模型旁证~\citep{videophy2}。
随后我们提出一个长期被忽视的问题：这些指标与人的判断一致吗？

\paragraph{指标审计。}
\label{sec:step2}
多数指标与人工标注的相关性很弱，$|\mathrm{SRCC}| \le 0.2$。
美学与画质类指标的退化尤为严重：十四项面向摄影的指标给出负相关，
而 AIGC 专用的感知模型也停留在 $0.2$ 以下。
它们的失效源于先验不同：照片域指标预设的是真实世界的照片，
而 AIGC 模型把短剧固有的风格化当成异常偏离（\cref{sec:audit}）。
本基准进一步弃用了三个叶子维度（含 \dc{V-D2}），它们的人工基线接近随机。
把自动化判分器对齐到近似随机的参照上，得到的结果无法解释。

\paragraph{多工具 agentic 判分。}
在此背景下，\judger{} 只保留那些相关性不可忽略、
且能提供大模型不具备的底层感知信号的指标，把它们用作辅助线索而不是直接的打分输入。
每个叶子维度独立且并发地跑多轮 agentic 打分。
系统会为每个目标维度自动路由相关度量；agent 还可以额外调用感知工具（局部放大、按时间戳截帧），
在依据逐题核查清单打分之前做细粒度查验。
输出的判定包含取自标注员的缺陷标签与时空定位，
因此一旦出现模型与人的分歧，可以直接交叉核对。
\cref{fig:judgemap} 给出各粒度上实际运行的核查项，\cref{fig:judge} 给出一个逐字段的判定示例。

\input{figures/fig_judgemap}

\input{figures/fig_judge}

\paragraph{采用的模型与配置。}
\label{sec:judgeconfig}
我们针对各环节各自的瓶颈采用不同的打分配置。
分镜设计取两个判分模型的输出均值，以降低对单一模型系列的依赖：
一个是 \md{gpt-5.6-sol-xhigh}，另一个是 \md{claude-fable-5} 的一个变体。
分镜图评测以 \md{doubao-seed-2.1-pro} 为主判分模型，
分镜视频评测采用 \md{gemini-3.1-pro}。


==> sections_zh/05_ablation.tex <==
\paragraph{实验设置。}
我们比较四种提示式架构：完整系统、去掉路由而来的小模型证据、去掉可调用工具，以及两者都去掉（纯 LMM）。
仅用测量值打分与训练得到的判分模型作为两条独立的基线。测试子集包含来自七个生成模型的 $210$ 张分镜图，
以及来自六个生成模型的 $180$ 条分镜视频。

\paragraph{感知与工具使用带来互补的增益。}
\cref{tab:ablation} 在 $14$ 个「模型--范式」单元上以 PLCC/SRCC 比较自动化均分与人工均分；
视频维度为各组共用，分镜图维度的覆盖随组别而定。在各环节的提示式判分模型固定的条件下（\cref{sec:judgeconfig}），
去掉路由证据或去掉工具，会使分镜图的 PLCC 分别从 $0.937$ 降到 $0.903$ 或 $0.891$；
视频的 PLCC 则从 $0.800$ 降到 $0.701$ 或 $0.656$。完整系统在分镜图（$0.880$、$0.677$）与视频（$0.445$、$0.632$）上
也都超过纯 LMM 与仅用测量值两条基线。这一模式与各组件的互补分工相符：
小模型提供感知证据，工具支持有针对性的检查，LMM 再把这些证据转化为依据判据的分数。

\paragraph{训练带来了本文报告的最高一致性。}
训练得到的判分模型在两组中都取得最高的 PLCC 与 SRCC：分镜图为 $0.955/0.912$，视频为 $0.851/0.837$。
它基于开源权重模型，只接收生成输入、待评产物与评分判据，不使用路由测量或工具，
却在分镜图与视频上分别比完整系统高出 $0.018$ 与 $0.051$ 的 PLCC。
两种相关系数上的提升都与「从标注样本中学到判据特定的分数校准与缺陷线索」相符，
而不是只依赖指令本身。

\input{figures/tab_ablation}


==> sections_zh/05_findings.tex <==
\paragraph{标注轮次时的最强链路。}
\label{sec:sota}
在有人工标注的模型中，按自动化评分，评测到的最强链路是：分镜用 \md{gpt-5.5-xhigh}、
分镜图用 \md{gpt-image-2}、视频用 \md{seedance-2.0}。
在同一模态内部，领先的已标注模型不随评测粒度改变：\md{gpt-image-2} 在两档分镜图上都居首（$3.99$、$3.82$），
\md{seedance-2.0} 在三档视频上都居首（$3.24$、$3.11$、$3.30$）。
这条链路运行在可用线附近：它的成片自动化得分为 $3.30$ 分，只比该线高 $0.3$ 分，
最好的单条 clip 是 $3.24$ 分。也就是说，已标注模型中最强的链路只是勉强达标，安全余量很小。
纳入标注轮次之后补测的模型后，\md{gpt-6-astra-max} 领跑分镜，\md{gpt-image-2.5} 领跑两档分镜图；
\md{seedance-2.0} 仍领跑分镜视频，而 \md{seedance-2.5} 的自动化成片得分最高（$3.70$），
并与 \md{wan-3.0} 并列集分镜视频最高分（$3.25$）。

\paragraph{分数沿文本到视频的链路逐环节下降。}
\label{sec:collapse}
在有人工标注的模型中，自动化平均分沿链路递减：分镜设计 $3.78$、单分镜图 $3.62$、集分镜图 $3.30$、
分镜视频 $3.09$、集分镜视频 $2.93$，到最终成片小幅回升至 $3.03$。
任何像素或视频生成环节都没有达到文本环节的 $3.78$ 分均值，
三档视频都落在可用线上下 $0.1$ 分之内，其中集分镜视频低于该线。
这一下降与两个因素相符。一是生成难度随产物获得像素、时序动态与声音而不断上升，
同一个评测角度被施加在越来越难的下游产物上。
二是缺陷会传导而不是停留在本地：每一环消费的都是上一环的产物，
而没有任何一个环节有权修复它继承来的问题（\cref{sec:prop}）。

\paragraph{判据有明确参照锚点时，基准的区分力最强。}
\label{sec:gaps}
在各轴适用的环节上取平均，自动化评分的首尾差为 \axF{} 输入保真 $1.22$、\axC{} 内部一致 $0.70$、
\axQ{} 视觉质量 $0.64$、\axP{} 生成合理 $0.53$、\axE{} 影视表现力 $0.42$。
这个次序与参照的明确程度相符：\axF{} 对着上游产物校验，\axC{} 对着同批产物校验，
而 \axP{}、\axQ{}、\axE{} 没有外部参照。锚点明确时，自动化基准的区分力看起来最强，
因此弱锚点指标上的小差距可能反映的是基准的局限，而不是模型表现相当。
人工标注支持这个判断，但次序并不相同：人工同样在 \axF{} 上分化最大，
而 \axE{} 在人工口径下是第二宽的一条轴，在本榜上却排在最后。

\paragraph{不同模型擅长的维度各不相同。}
\label{sec:profiles}
综合分掩盖了维度之间的取舍。单分镜图上，\md{seedream-5.0-pro} 与 \md{nano-banana-pro}
的自动化综合分只差 $0.02$，但前者在 \axF{} 输入保真上领先 $0.39$、在 \axP{} 生成合理上落后 $0.60$。
分镜视频上，\md{kling-3.0-omni} 与 \md{pixverse-c1} 综合分仅差 $0.01$，
而 \md{kling-3.0-omni} 在 \axP{} 上高 $0.16$、在 \axE{} 影视表现力上低 $0.22$。
两对模型的逐维差距都比综合分差距大一个数量级。
所以综合分适合分档，却会误导选型：该问的是「在哪一维上更好」，而不是「哪个模型更好」。
具体案例见 \cref{app:cases}。


==> sections_zh/05_validation.tex <==
\label{sec:meta}
\label{sec:meta-agree}
\label{sec:meta-axis}
\label{sec:meta-rank}
\label{sec:meta-fail}
\label{sec:hbdef}

\input{figures/tab_agree}

\paragraph{与人工参照的一致性。}
参考集中的全部 $5{,}569$ 道题都有三名标注员的独立标注，为后续的相关性分析建立了两个层面的参照基准。
在模型级上，参照标准是三人共识所导出的排名，相关性直接对这一人工排名计算。
在逐题层面上，评估依据的是逐题共识分，并采用留一法人工基线（\hbase，
即取一名标注员去预测另外两人的均分，三人轮换后汇总），
以排除脱离判据可复现程度、因而无效的绝对相关结果。详细推导与实例见 \cref{app:agreeslices}。
两个层面的一致性分析表明，模型级的一致性是稳健的：自动化评测在六个环节上的 PLCC 均值为 $0.918$，
在短剧成片上自动化排名与人工排名完全对齐（SRCC $= 1.000$）。
\cref{tab:main} 中另外十五个模型依赖的正是这一模型级一致性：它们仅由自动化评测打分，本身并未与人工评分核对。
在逐题层面上，一致性表现则随链路环节明显分化：文本与图像环节达到或超过人工基线，
其中分镜设计达到基线的 $2.35$ 倍，但分镜环节有几个维度的人工基线本身就很低（\cref{sec:storyboard}）；
相比之下，三档视频落到基线的 $0.79$--$0.85$ 倍：相关性仍为正，但逐题一致性低于标注员彼此之间的一致性。

\paragraph{一致性由什么决定。}
人机一致性沿环节的分化，与评测任务的两项属性相符，而与判据的主观性无关。
其一，评测模态决定一致性表现：关键的分界落在静态图像与动态视频两种模态之间，
而不是落在单条与多条素材之间（\cref{fig:ratio}）。
集分镜图评分需要认知负担更重的跨帧比对，却达到基线的 $1.48$ 倍；
而孤立评判一条视频 clip 只有基线的 $0.79$ 倍。
按模态归并，自动化打分的一致性稳定衰减：文本 $0.509$、像素图像 $0.440$、时序与音轨内容 $0.296$；
而人工标注员之间的一致性在这三种模态上反而上升（$0.217$、$0.341$、$0.357$），
呈现出一个相反的趋势：自动化评测最差的场景，恰恰是人类共识最高的场景。
其二，有没有外部校验参照，决定了各评测轴之间的层级差距（\cref{tab:axes}）：
一致性依次为 \axF{}（$0.423$）、\axC{}（$0.235$）、\axP{}（$0.146$）、\axE{}（$0.132$）、\axQ{}（$0.121$）。
只有 \axF{} 相对人工基线取得净提升（$+0.107$，$12$ 项中有 $9$ 项占优），
而 \axQ{} 在它的四项测试里一项都没有超过基线。

\input{figures/fig_ratio}

\paragraph{人机一致性的预测因子。}
\label{sec:quadrant}
按常规预期，人机一致性应当随判据主观性升高而下降；
但本研究观察到的是相反的形态：主观性与自动化打分误差之间并无正相关。
最主观的维度（视听风格处理）达到基线的 $6.5$ 倍，但这一倍数被接近于零的人工基线放大了；
而表现最差的几个维度（画质、运动平滑、环境物理、声画同步）全都是客观指标。
比主观性更贴合一致性高低的，是两项落在任务层面的属性：
判据能否被拆解为可枚举的检查项，以及判定是否需要细粒度的感知分辨（\cref{tab:quadrant}）。

\input{figures/tab_quadrant}


==> sections_zh/06_judgetrain.tex <==
\paragraph{训练数据。}
训练样本把基准产物与人工均分及相应的归因文本配对。分歧较大的标签会被降权或剔除。
低分题与指令不匹配的负样本扩展了分数的覆盖范围，通用视频样本则用于补充视频判分模型的训练。
\cref{sec:ablation} 中的测试子集在监督微调（SFT）与 GRPO 两个阶段都被留出。

\paragraph{训练算法。}
我们微调两个开源权重模型，并冻结各模态编码器：视频用 \md{Qwen3-Omni-30B-A3B}，分镜图与分镜脚本用 \md{Qwen3.8-27B}。
SFT 通过 token、分数回归与指令遵循三类目标学习结构化理由与判据分数。
分数是五个档位 token 上的连续期望，$\hat{s}_{d}=\sum_b v_b p^{(d)}_b$，其中 $v_b\in\{1,\ldots,5\}$，
$p^{(d)}_b$ 为维度 $d$ 上档位 $b$ 经重新归一化后的概率。GRPO 随后优化奖励
\begin{equation}
R \;=\; R_{\text{score}} + 0.2\,R_{\text{fmt}} + 0.3\,R_{\text{attr}},
\label{eq:reward}
\end{equation}
\begin{equation}
R_{\text{score}} \;=\; \sum_{\ell \in \{1,2\}} \omega_{\ell}
  \operatorname{mean}_{d \in \mathcal{D}_{\ell}}
  \big[\,1 - \tfrac{1}{4}|\hat{s}_{d} - s^{\ast}_{d}|\,\big]_{+} ,
\label{eq:rscore}
\end{equation}
其中 $s^{\ast}_{d}$ 为人工目标分，$(\omega_1,\omega_2)=(0.6,0.4)$ 分别是轴级维度 $\mathcal{D}_1$ 及其叶子维度
$\mathcal{D}_2$ 的权重。$R_{\text{fmt}}$ 检查输出格式；$R_{\text{attr}}$ 把预测的定位与标签和已有的人工标记比对。
因此，奖励综合了分数一致性、格式合规与缺陷归因。\cref{app:train} 概述了各模态的监督方式与推理耗时。


==> sections_zh/06_results.tex <==
\section{实验}
\label{sec:results}

\subsection{实验设置}
\label{sec:setup}

$9$ 个文本大语言模型、$7$ 个图像模型和 $6$ 个视频模型通过人工标注和自动化评测完成打分；
另有 $15$ 个新模型（$11$ 个文本、$1$ 个图像、$3$ 个视频）仅使用自动化评测，在相同的题面上完成评测，
对应 \cref{tab:main} 中标 $\dagger$ 的行；其中 \md{wan-3.0} 与 \md{seedance-2.5} 使用更长的时长预算并重新规划分镜，
其单元按剧、集、范式与镜号对齐（\cref{sec:cov}）。
评测分值满分为 $5$ 分，\textbf{\boldmath $3.0$ 分为可用／需返工的分界阈值}。模型名沿用各厂商自己的写法；
结尾的 \texttt{-xhigh}、\texttt{-max} 或 \texttt{-high} 是该次运行采用的推理档设置，并非名称的一部分。
因为模型侧审核与生成失败等问题，部分模型无法生成全部题：这些模型按其实际跑过的切面计分，
在 \cref{tab:main} 中以 $\ddagger$ 标出；缺口逐项列在 \cref{sec:cov}。
主表、模型排名与分环节描述使用自动化评分；人工评分在文中注明。

\subsection{主要结果}
\label{sec:mainresults}
\label{sec:leaderboard}
\label{sec:quant}

\input{figures/tab_main}

\cref{tab:main} 是六个环节全部的自动化榜，并按五条评测轴展开。

\input{sections_zh/05_findings}

\subsection{一致性检验}
\label{sec:align}

\input{sections_zh/05_validation}

\subsection{训练判分模型}
\label{sec:judgetrain}

\input{sections_zh/06_judgetrain}

\subsection{消融实验}
\label{sec:ablation}

\input{sections_zh/05_ablation}

\subsection{分环节分析}
\label{sec:perstage}

\noindent
下面三部分对应链路的三种\emph{模态}而不是单个粒度，合起来覆盖全部六个：
分镜设计是 \textcircled{1}，即文本环节；分镜图覆盖 \textcircled{2} 与 \textcircled{3}；
分镜视频覆盖 \textcircled{4} 至 \textcircled{6}。

\input{sections_zh/06_stage_storyboard}
\input{sections_zh/07_stage_image}
\input{sections_zh/08_stage_video}

\input{sections_zh/07_discussion}


==> sections_zh/06_stage_storyboard.tex <==
\subsubsection{分镜设计}
\label{sec:storyboard}

被评对象是把分集剧本改写成分镜脚本的 $9$ 个文本大语言模型，共 $533$ 道评测题。
九个模型的自动化得分区间为 $3.26$--$4.23$（\cref{tab:main}），
是三个单条粒度任务中差距最大的一档。标注轮次结束之后，另有十一个模型在同一批题面上完成了评测。

\input{figures/tab_sbdims}

\paragraph{性能瓶颈落在可调度的制作缺陷上。}
按自动化均分，八个叶子维度中有七个达到可用线，其中六个得分在 $3.89$ 与 $4.18$ 之间，
说明模型能够忠实复现剧本的核心要素：情节事件、人物台词与场景呈现。
得分最低的两个维度都决定制作逻辑：拍摄节奏 $2.74$、增补克制 $3.34$（\cref{tab:sbdims}）。
文本分镜环节的瓶颈在于制作调度与时长预算，而不在语言生成能力。
时长预算遵循可量化的算术规则，在任何画面被渲染之前就能完成核验，
因此这一环节的主导缺陷可以在前期制作阶段识别并纠正。

新增模型中有九个在对比中有同一家族的上一代模型。九个的自动化得分均高于各自的上一代，增幅为 $+0.02$ 至 $+0.60$；
最新的 \md{gpt-6-astra-max} 以 $4.43$ 分居本环节最高。

\paragraph{一致性倍数取决于人工可复现性。}
逐题一致性为 $0.509$，人工基线为 $0.217$（$2.35$ 倍），且每一个维度都超过其自身基线（\cref{tab:sbdims}）。
基线倍数反映的是人工可复现性的差异，而不单是自动化评分的表现。
对白保真可以逐字对着剧本核验，自动化评分与人工两侧的一致性都高（$0.728$ 对 $0.442$）；
相比之下，视听风格处理的倍数最大，为 $6.5$ 倍，但其自动化一致性只有 $0.265$，
倍数之所以大，是因为人工基线仅为 $0.041$：标注员彼此之间也几乎无法对齐。
增补克制的基线为 $-0.023$，倍数无法解释。
只有在人工判据本身可复现时，大的倍数才支持「可自动化」；否则，更高的自动化一致性并不能证明其有效。
这些维度仍需要更清晰的可操作判据（\cref{tab:quadrant}）。

\paragraph{新增模型仅由自动化评测打分。}
十一个新增模型以分轴得分进入 \cref{tab:main}，没有各自的一致性统计，增量人工标注成本为零。
它们的分数是把在已标注模型上校验过的判分系统延伸过去得到的，本身并未与人工评分核对。


==> sections_zh/07_discussion.tex <==
\subsection{全链路分析}
\label{sec:discussion}
\label{sec:chain}

\paragraph{上游缺陷会沿生成链路向下传导。}
\label{sec:prop}

\input{figures/fig_prop}

如果视频生成环节构成主要瓶颈，那么替换上游模型对成片的影响应当微乎其微；
实际观察到的却是显著变化。在视频模型固定的条件下，我们只把一个上游环节换成更弱的模型：
分镜环节换成 \md{hy3} 或 \md{mimo-v2.5-pro}，图像环节换成 \md{nano-banana-pro} 或
\md{seedream-5.0-lite}；在四部剧、首尾帧范式下共得四种替换，各自在三个粒度上读取，
并与由有人工标注的头名模型组成的基线链路对照，真人剧改用 \md{happyhorse-1.1}，
因为 \md{seedance-2.0} 不覆盖真人剧（\cref{sec:degrade}）。
按自动化评分，只替换一个环节，就使单条 clip 的质量下降 $0.07$--$0.13$ 分、
连续片段下降 $0.06$--$0.37$ 分、成片下降 $0.25$--$0.83$ 分（\cref{fig:prop}）；这些替换链路由自动化评测打分，没有人工标注。
测得的质量损害随时间观测窗口的变宽而放大，
因为上游环节所作的决定是不可逆的，任何下游模块都无法推翻。

\paragraph{判分粒度会改变评测分数。}
\label{sec:unit}
单个产物在孤立评测时往往能拿到不错的分数，
但把这些独立的帧与镜头拼接成连续片段或整集之后，
跨帧的隐性不一致会不断累积，使整体得分急剧下降。
按三名标注员的均分，一集的分镜图逐张判时得分为 $3.33$--$4.00$，作为一组来判只有 $2.33$；
一集的分镜视频中被单独评过的那些镜头得分在 $3.23$ 至 $4.00$ 之间，连成一段却只有 $1.67$，
而扣分全部来自跨镜的人物呈现、场景道具对齐与动作连贯性上的错配（\cref{fig:unit}）。
同样的粒度落差在全语料上同样成立：角色外观、场景道具、动作连贯与语音质量等各项的人工分，
从分镜级到集级评测都下降接近一整档。
因此单条基准忽略了累积性的跨帧不一致，测的是一个孤立的量，
它无法作为整集生成质量的有效代理。

\input{figures/fig_unit}

\paragraph{自动化的局限与模态相关。}
\label{sec:modality}
按模态取均值，逐题一致性沿生成链路下降（文本 $0.509$、像素 $0.440$、时序与音轨 $0.296$；\cref{sec:align}），
这表面上容易被读成「越靠后的环节越难评」。
但按评测轴与数据模态做分解之后，这一下降主要随模态而变，而不是随环节而变（\cref{tab:axismod}）。
纵向读，\axF{} 输入保真在每一种模态下都表现最强；
横向读，随着模态依次纳入像素、时序与音频，除 \axP{} 之外的每一条轴都在退化。
两个因素的作用看起来是叠加的。一个有代表性的例子是 \axE{} 影视表现力：
同一项要求写进分镜脚本时，四个维度全部达到人工基线；
而当它被渲染为视频时，十一个维度中没有一个达到。
下游环节并没有引入更主观的判据，而是评估所需的证据在感知上变得更难提取，
这提示对症的是补感知能力，而不是调提示词。

\input{figures/tab_axismod}

\paragraph{归因需要真实的上游产物。}
本文的每一道题都由链路实跑产出、且只在被测环节分叉，
因此每一处缺陷都能被记到产生它的那个环节名下，而不是记到最后经手它的那个环节：
把三个人的对话压进同一个镜头、使谁说哪一句只能由视频模型自行推断的那份分镜，
以及让场景先于人物漂移的那批分镜图，都被记在分镜设计与分镜图这两环上。
这正是跑通整条链路换来的东西，也是本节全部结论所依赖的性质。


==> sections_zh/07_stage_image.tex <==
\subsubsection{分镜图}
\label{sec:image}

被评对象是把分镜脚本画成关键帧的 $7$ 个图像模型，共 $2{,}125$ 道单张题与 $429$ 道集级题。
各模型在单张任务上的得分相近；人工综合分在集级分镜图这一档首次跌破可用线（$2.74$；\cref{tab:imgdims}）。

\paragraph{短板集中在「把指定内容放对位置」上。}
按自动化均分，十五个单张维度中有三个跌破可用线，而这三个问的都是「链路已经指定过的内容有没有被放对」：
主体属性对角色设定卡（$2.75$）、场景对参考图（$2.72$）、镜头构图与视觉风格对分镜描述（$2.91$）。
这一类之外没有任何维度失守：十五个维度铺开在 $2.72$--$4.59$，
而两个画质维度、两个生成合理维度与风格一致维度都在线以上（\cref{tab:imgdims}）。
制约单张环节的是对规格的遵循，而不是把画面画出来的能力，
这把改进的着力点定位在条件注入与参考素材的处理上，而不是渲染能力上。

\paragraph{跨镜一致最先失守。}
按自动化均分，四个集级维度中有两个跌破可用线，而其中更低的那个并不符合直觉：
场景一致（$2.50$）比角色一致（$2.87$）更差。
场景分更低，反映的是布局、陈设与光线的变化，而不是演员本身的改变（\cref{tab:imgdims}）。
当同一批分镜图被当作一整集来评时，退化的是画面中各实体的\emph{持续性}，
而不是任何单帧的观感。这一持续性正是单张评测看不见的性质。

\paragraph{综合分接近掩盖了完全不同的能力构成。}
\label{sec:closepairs}
本榜上综合分相差不超过 $0.03$ 分的模型只有一对，
它说明了 \cref{sec:profiles} 提出的轴级能力结构。
\md{seedream-5.0-pro} 与 \md{nano-banana-pro} 的自动化综合分只差 $0.02$，
而前者在 \axF{} 输入保真上领先 $0.39$、在 \axP{} 生成合理上落后 $0.60$：
轴级差距比综合分差距大一个数量级。
强项是沿整条能力轴出现的，而不是零散分布在各个维度上。
因此综合分足以用来分档，却会在按具体生产需求选型时产生误导。

\paragraph{题面提供明确参照时，自动化一致性更高。}
常规认知是客观判据容易自动化、主观判据难自动化，而这一环并不按这条线分开。
十五个单张维度中有九个达到或超过人工基线，四个集级维度全部达到；
而缺口显著的四个恰好是 \axQ{} 与 \axP{} 的全部四项（\cref{tab:imgdims}）。
其中画面质感、人体结构与环境物理，正是整个维度体系里物理意义上最客观的三项。
区分结果的似乎是题面有没有给出答案，而不是判据听起来有多客观。
画面质感看上去是十五个维度里最可度量的一个，
但一帧偏柔、偏灰的画面，既可能是没拍清楚，也同样可能是这部剧要的质感，
题面里没有任何东西能判定它要的是哪一种：自动化判分器只有 $0.167$，对应基线 $0.275$。
动作交互是一项「画面里正在发生什么」的判断，却是本环节被服务得最好的维度，
以 $0.527$ 对 $0.401$，因为分镜描述写明了应该发生什么。

\input{figures/tab_imgdims}


==> sections_zh/08_conclusion.tex <==
\section{结论}
\label{sec:conclusion}

短剧生成是一条由数个环节串起来的链路。\bench{} 对这条链路的每一环打分，
所用题面均由链路自身产出。这一设计使缺陷能够被归到产生它的那个环节，
而不是归到仅仅观察到它的那个环节。支撑它的是三套自建系统：\pipe{}，
一条生成流程与成片质量对标商用短剧平台的产线，所有题面由它产出，且只在被测环节分叉；
\labeler{}，专业标注员在其中对每道题的每个适用维度打分，
扣分在适用时进行时空定位、并从固定词表中取归因；以及 \judger{}，
一个在用于给模型排名之前先对着这份人工参照完成校验的 agentic 自动化判分器。

比起当作排行榜，我们更希望 \bench{} 被当作一份诊断来用。
产线、维度体系与判分配置都可以按现状复用：
新模型可以接入任意单一环节并由自动化评测打分，但这些分数本身并未与人工评分核对；
而仍然依赖人的那些部分被明确暴露出来，而不是被掩盖。
我们鼓励后续工作把评测放在短剧生产真正失效的地方：环节与环节的交界处，
以及一集之内的若干镜头之间，而不是孤立地评测单条片段。


==> sections_zh/08_stage_video.tex <==
\subsubsection{分镜视频与短剧成片}
\label{sec:video}

被评对象是把关键帧生成为视频、并把结果连成整集的 $6$ 个视频模型，
共 $2{,}186$ 道分镜级题、$306$ 道集分镜视频题与 $206$ 道成片题。
在自动化榜上，有人工标注模型的首尾差从分镜级的 $0.36$ 分扩大到成片的 $0.51$ 分。

\paragraph{最弱的那些维度，都是随时间展开的。}
按自动化均分，本环节二十个叶子维度的得分区间为 $1.49$ 至 $4.15$（\cref{tab:viddims}）。
声画同步得分最低，为 $1.49$，人物表演同样处在末段，为 $2.34$；
得分最高的三个则是风格一致（$4.15$）、帧图遵循（$4.14$）与画面质感（$4.11$）。
区分两端的判据在于：该维度考察的是画面的静态观感，还是片段随时间展开的动态行为，
而模型在后者上表现最差。这一类缺陷是任何静态图像基准都无法检出的。

\input{figures/tab_viddims}

\paragraph{判分单元变粗，数的就是另一类缺陷。}
同时定义在分镜级与集级两个粒度上的十个维度中，有四个考察跨镜一致性，
而随着判分单元变粗，这四个维度的自动化均分全部下降：
风格一致由 $4.15$ 降至 $3.32$、动作一致由 $2.56$ 降至 $1.93$、
场景道具一致由 $2.33$ 降至 $1.82$、角色外观一致由 $3.44$ 降至 $3.21$（\cref{fig:granularity}）。
扣分所对应的缺陷类型同样发生了实质变化：
分镜级上的扣分指向的是这一条片段本身的执行错误，
集分镜视频上的扣分反映的是同一集内各片段之间的不匹配，
而成片上的扣分对应的是整集自行虚构的叙事内容。这一缺陷类别在分镜级评测中完全不存在。
判分单元变粗，重塑的是可被检出的缺陷谱系，而不只是改变了缺陷的数量，
因此局限于单条片段的评测结果，无法外推到短剧成片的交付标准。

\input{figures/fig_granularity}

\paragraph{输入约束塑造了各范式的强项。}
在分镜级评测上没有任何一种范式取得绝对优势，
而每一种范式的表现构成，都由它的输入约束机制决定（\cref{tab:paradigm}）。
宫格范式把多个镜头整合进同一张图像，使各镜头共享人物主体与场景背景的像素信息，
因此在人景融合（$4.28$）、角色外观一致（$3.67$）与风格一致（$4.32$）上都取得最好成绩；
但每一镜对应的是该图像中的一个局部单元，而不是一帧属于自己的完整画面，
于是对单元的遵循（$3.97$）低于对首尾帧对的遵循（$4.28$）。
首尾帧范式为每一镜提供首末两个关键帧，因而在帧图遵循（$4.28$）上占优，
这也正是它的输入唯一钉死的那条性质；它对中间内容不施加任何约束，
于是在人景融合（$3.01$）与镜头运动（$3.30$）上得分最低。
多参考范式无需复现固定帧，镜头因此获得自由，取得最高的镜头运动合理性（$4.09$）
与最好的音效配乐（$3.62$）；而固定视觉锚点的缺失，使它在风格一致上垫底（$4.04$），
但只落后 $0.28$ 分。
每种范式取得的特定强项，都源自它选择放弃的那条输入约束，
这说明输入格式是一项影响实际表现的部署决策，而不是无关紧要的实现细节（\cref{app:paradigmcase}）。

\input{figures/tab_paradigm}

\paragraph{参照是否存在，对视频同样重要。}
该规律在这里同样成立，衡量它的是逐题一致性而不是均分。
可对着剧本事件清单核对的事件完成度达到 $0.363$，对应基线 $0.200$；
而不存在文本参照的成片可看性只有 $0.074$，对应基线 $0.343$（\cref{tab:viddims}）。
这一环还为该规律提供了一组近乎受控的对照：
语音质量与声画同步共享模态、共享工具链，人工基线也相当（$0.474$ 与 $0.448$），
自动化判分器在前者上达到 $0.354$，在后者上却只有 $0.075$。
主要差别在于：剧本台词为语音质量的评测提供了明确的文本锚点，而声画同步不存在这样的参照。
在分镜级上，声画同步既是得分最低的维度，也是相对自身人工基线差距最大的维度（$0.17$ 倍），
因此它的位置记录的是自动化判分器的能力上限，而不是各生成模型之间的相对排名。


==> sections_zh/09_ethics.tex <==
\section*{伦理与负责任使用}
\phantomsection
\label{sec:ethics}
\addcontentsline{toc}{section}{伦理与负责任使用}

本基准的全部产物都是生成的：剧本为本项目原创，所有角色设定卡、分镜图与视频片段都是模型输出，
没有使用任何真人的肖像、声音或商业短剧素材；三个商用平台（\cref{sec:sourcing}）通过公开接口运行我们的剧本。
语料带有短剧常见的冲突、胁迫与复仇等母题；所有题面都按商业上线的内容政策做过筛查，但没有做更广义的危害审计。
标注由第三方供应商的专业签约人员完成（\cref{sec:annot}），报酬按供应商条款执行。
本基准用于逐环节比较生成模型与诊断缺陷，不能预测商业表现（\cref{tab:scope}），也不评测安全或内容政策。


==> sections_zh/10_limitations.tex <==
\section{局限}
\label{sec:limitations}

每个模型级相关系数只基于六到九个有人工标注的模型，而且有若干叶子维度的人工可复现性偏低（\cref{sec:slice-consensus}），
削弱了它们作为对齐目标的价值。\label{sec:cov}覆盖面也不完整且并非随机：模型侧的内容审核与生成失败，
使 \md{seedream-5.0-lite} 只覆盖 $20$ 部剧中的 $10$ 部，\md{veo-3.1} 与 \md{wan2.7} 只覆盖首尾帧范式，
\md{seedance-2.0} 只覆盖动画，\md{seedance-2.5} 只覆盖动画多参考条目；这些模型（\cref{tab:main} 中的 $\ddagger$）
按其实际产出的条目计分。时长预算也有差异：\md{wan-3.0} 与 \md{seedance-2.5}（$30$\,秒，重新规划分镜）以及 \md{veo-3.1}（$10$\,秒）
按剧、集、范式与镜号对齐。
一个 $63$ 维的体系容易让人以为它是穷尽的，因此\cref{tab:scope} 明确列出本基准的负向覆盖。

\input{figures/tab_scope}


==> sections_zh/11_ack.tex <==
\section*{致谢}
\phantomsection
\label{sec:ack}
\addcontentsline{toc}{section}{致谢}

衷心感谢河套学院的李云鑫老师、户保田老师、张民老师，北京大学的向勇老师，
北京电影学院的洪帆老师，深圳大学的高飞老师对本文的支持。
也特别感谢导演专家徐烨凯、黄天伦，编剧专家李彦仪，制片专家黄家后，美术专家袁佳欣，
摄影专家陈想、李佳雨、汤子晨，剪辑专家张宁轩，调色专家蒋尚恒在影视方面提供的专业意见。
感谢腾讯的彭湖鑫、董梁在数据采购上的帮助。


==> sections_zh/A_dimensions.tex <==
\section{维度体系及其实现}
\label{app:dims}

\dimsys{} 定义了 $66$ 个叶子维度，本报告评的 $63$ 个是这 $66$ 个减去三个
因人工基线接近零而弃用的维度（\cref{sec:step2}）。每个叶子维度另配五档可判定描述与一组归因标签，
人工与自动化共用；标签词表见 \cref{sec:tagvocab}，五档描述篇幅所限不在此重列。
逐维度的分数与一致性见 \cref{sec:perstage} 的各环节分表。

\label{app:impl}
\label{app:tools}
\label{app:steps}

\subsection{每个叶子维度的实现}
\label{sec:impl}

每个叶子维度的实现方式是同一套，而且整套都是声明式的。schema 里一个维度的条目带三样东西：
五档判据、一份封闭的标签词表，以及一行说明「要核什么」的 \emph{method}；
路由器会扫描这一行的关键词并挂上它点到的取证 producer，
所以「这个维度被定义为核什么」直接决定了「为它测什么」，没有任何逐维度的代码。
证据随后通过两条路径到达自动化评测。
\textbf{路由度量}无条件运行：每个维度用到 $29$ 个 producer 中的零到三个。
\textbf{可自调用工具}可以多轮自行调用，只有声明了它们的维度才拿得到，因此注册表里 $17$ 个中有 $15$ 个
真正可达。没有任何 \texttt{pixel\_sensitive} 维度声明含改像素工具的集合，路由在那里也会把它们扣下，
所以画质永远不会在一张修过的帧上被评。打分随后给出档位、取自该维度标签表的标签，以及理由。

表格读法：\textbf{实现方式}是对路由器所读的那行 method 的转述；
\textbf{路由取证}是 \texttt{route\_tools} 为它选中的工具，由执行路由逻辑追踪得到，而不是照读配置，
「---」表示它没有为该维度选中任何 producer；
\textbf{可自调用工具}是解析后的工具集，「---」标记的是无法按需看得更细的维度。
叶子维度名称沿用 \cref{app:dims}，工具名为简写，全称见 \cref{tab:tools}。
标\fail{空转}的是：路由挂上了该 producer，但它在该环节的每道题上都返回不可用，
因此这一维度实际由判分模型单独打出。\dc{S-C4} 的 method 行提到 CSD，而 CSD 是图像模型、
分镜环节没有像素；\tl{identity\_sim} 在跨镜与整集上被暂停，因为那里的身份匹配常把一个角色拆成两个、
或把两个并成一个。另有一个 producer 完全不走路由：\tl{cut\_detect} 在每条视频或整集题上算一次，
随基础上下文进入每一条 prompt。

「可自调用工具」列给出的是 schema 为该维度声明的工具集名，括号内数字为集内工具数。
\tl{detail(2)} 为 \tl{zoom\_in} 与 \tl{draw\_bbox}；\tl{count(3)} 与 \tl{scene(3)} 在其上再加
\tl{count\_marker}；\tl{fine(4)} 则改为再加 \tl{sharpen} 与 \tl{super\_resolution}，
\tl{lowlight(4)} 再加 \tl{enhance\_contrast}。
视频侧的每个集都以 \tl{video\_probe} 与 \tl{extract\_frame} 起头，
因为视频在抽出一帧之前没有可放大的静态图：\tl{v\_frame(4)} 在其上加 \tl{zoom\_in} 与 \tl{draw\_bbox}，
\tl{v\_count(5)}、\tl{v\_text(5)} 与 \tl{v\_cut(5)} 分别再加 \tl{count\_marker}、\tl{ocr\_frame}
与 \tl{detect\_scenes}，\tl{v\_sync(5)}、\tl{v\_audio(4)} 与 \tl{v\_speech(7)} 则围绕音频工具组装，
并去掉它们用不上的标注与放大工具。
全部工具的全称见 \cref{tab:tools}。

\subsection*{\textcircled{1} 分镜设计}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{S-A1} & 事件覆盖 & \axF{} & 主 agent 抽剧情节点 → 子 agent 逐镜对齐算覆盖率 & \tl{event\_align} & \textcolor{rulegray}{---} \\
\dc{S-A2} & 对白保真 & \axF{} & 对白文本对齐（编辑距离 + 嵌入相似度） & \tl{dialogue\_align} & \textcolor{rulegray}{---} \\
\dc{S-B1} & 描述可执行性 & \axP{} & VLM 分表述清晰 / 承载可解析 / 空间物理可行三项核查 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\dc{S-B2} & 补充适度性 & \axP{} & LLM 逐镜抽多余细节 + 转场衔接要素 + 关键补充缺口，再判是否越界或伤一致性 & \tl{supplement\_audit} & \textcolor{rulegray}{---} \\
\dc{S-C1} & 叙事流畅度 & \axE{} & LLM 抽跨场景硬切 + 段落内衔接断裂 + 镜内先后顺序 + OS 错位，按七类形态定档 & \tl{narrative\_flow\_audit} & \textcolor{rulegray}{---} \\
\dc{S-C2} & 拍摄节奏 & \axE{} & 统计单镜动作动词数与时长分布 + VLM 判可落地性 & \tl{shot\_stats} & \textcolor{rulegray}{---} \\
\dc{S-C3} & 情绪表达 & \axE{} & LLM 逐情绪节点抽视听八通道外化设计 + 导演校准 & \tl{emotion\_beats} & \textcolor{rulegray}{---} \\
\dc{S-C4} & 视听风格处理 & \axE{} & 镜头语言分类 + 剧种词表 + 导演校准 & \tl{style\_csd}\,\fail{（空转）} & \textcolor{rulegray}{---} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{2} 单分镜图}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{I-A1} & 技术质量 & \axQ{} & 放大核对三类瑕疵，清晰度为主导项 & \textcolor{rulegray}{---} & \tl{zoom(1)} \\
\dc{I-A2} & 美学风格 & \axQ{} & CSD 风格纯度 + 剧种词表，判色彩光影协调与廉价 AI 感 & \tl{style\_csd} & \textcolor{rulegray}{---} \\
\dc{I-B1} & 主体属性 & \axF{} & SAM 分割 + 放大逐 facet 判 0/1/2 & \tl{sam\_count} & \tl{count(3)} \\
\dc{I-B2} & 动作交互 & \axF{} & 逐 facet 判分 & \textcolor{rulegray}{---} & \tl{detail(2)} \\
\dc{I-B3} & 场景与空间布局 & \axF{} & 场景类型核对 + 输出方位程序比对 & \tl{scene\_consistency} & \tl{count(3)} \\
\dc{I-B4} & 镜头与视觉风格 & \axF{} & 镜头属性分类 + 构图与光影判定 + CSD 风格匹配 & \tl{style\_csd} \tl{framing\_check} & \textcolor{rulegray}{---} \\
\dc{I-C1} & 人脸身份 & \axF{} & 真人走 ArcFace；动漫脸走动漫识别或 DINOv3 通用特征相似度 + CIDS~\citep{dinov3,vistorybench}，由本文审计结果选用 & \tl{identity\_sim} & \tl{fine(4)} \\
\dc{I-C2} & 外观服饰 & \axF{} & 放大比对设定卡，配饰等小物件需放大 & \textcolor{rulegray}{---} & \tl{fine(4)} \\
\dc{I-C3} & 关键元素保真\,\fail{（已弃用）} & \axF{} & 道具区域 SAM 裁切 + 嵌入或 VLM 比对参考 & \tl{sam\_count} & \tl{detail(2)} \\
\dc{I-D1} & 角色跨图 & \axC{} & CIDS / DINOv3 通用特征两两相似度聚合 & \tl{identity\_sim} & \tl{fine(4)} \\
\dc{I-D2} & 人景融合度 & \axC{} & CPR~\citep{vistorybench} / NaturalScore~\citep{opens2v} + 判人景光影与透视融合，须与 I-D1 对抗评 & \tl{copypaste\_var} & \tl{detail(2)} \\
\dc{I-D3} & 场景及布局 & \axC{} & 场景库嵌入跨图一致 + 复核空间结构 & \tl{scene\_consistency} & \tl{scene(3)} \\
\dc{I-D4} & 轴线 & \axC{} & 输出每镜主体朝向与运动方向 + 规则比对越轴 & \tl{axis\_check} & \tl{detail(2)} \\
\dc{I-D5} & 风格一致性 & \axC{} & CSD 风格嵌入跨图一致，宫格拆子格后在子格间比 + 逐格检画风混搭 & \tl{style\_csd} & \tl{detail(2)} \\
\dc{I-E1} & 人体结构合理性 & \axP{} & 人体与手部关键点检测 + 放大核手部畸形，并判姿态自然度 & \tl{body\_structure} & \tl{count(3)} \\
\dc{I-E2} & 环境物理合理性 & \axP{} & 按重力 / 碰撞 / 透视 / 光影分项检测 & \textcolor{rulegray}{---} & \tl{detail(2)} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{3} 集分镜图}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{MI-D1} & 角色跨镜一致 & \axC{} & 跨镜两两身份相似度聚合 + gap-decay & \tl{identity\_sim}\,\fail{（空转）} & \tl{fine(4)} \\
\dc{MI-D2} & 人景融合度 & \axC{} & 跨镜构图相似度过高告警 + 判人景融合，与 MI-D1 对抗 & \tl{framing\_check} \tl{copypaste\_var} & \tl{detail(2)} \\
\dc{MI-D3} & 场景跨镜一致 & \axC{} & 场景库嵌入跨镜一致 + 放大逐件比对陈设 & \tl{scene\_consistency} & \tl{lowlight(4)} \\
\dc{MI-D4} & 空间方位连贯\,\fail{（已弃用）} & \axC{} & 输出每镜朝向与位置 + 估机位，规则比对越轴 & \tl{axis\_check} & \tl{detail(2)} \\
\dc{MI-D5} & 风格跨镜一致 & \axC{} & CSD 风格嵌入跨镜一致 + 逐段放大检画风突变，色调按场景分组 & \tl{style\_csd} & \tl{detail(2)} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{4} 分镜视频}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{V-A1} & 画质与材质 & \axQ{} & DOVER / MUSIQ 感知质量 + 拉普拉斯锐度 + 判材质是否贴合作品风格 & \tl{quality\_metric} & \tl{v\_frame(4)} \\
\dc{V-A2} & 美学画风与动态质感 & \axQ{} & 美学回归 + 判画风与剧种匹配；动态质感另据光流 & \tl{quality\_metric} \tl{aesthetic\_metric} \tl{style\_csd} & \textcolor{rulegray}{---} \\
\dc{V-B1} & 主体属性准确度 & \axF{} & 抽帧 + SAM + 目标检测计数，核满足率 & \tl{sam\_count} & \tl{v\_count(5)} \\
\dc{V-B2} & 镜头与视觉风格 & \axF{} & 镜头属性分类 + 构图与光影判定 + 镜头切换数 & \tl{framing\_check} & \tl{v\_frame(4)} \\
\dc{V-B3} & 帧图遵循 & \axF{} & 对应帧与给定帧 SSIM~\citep{ssim} / DINO + 主体框对齐 & \tl{frame\_follow} & \tl{v\_frame(4)} \\
\dc{V-C1} & 角色外观一致 & \axC{} & 逐帧特征一致与闪烁度 + 锚点 gap-decay + 服装比对，先过保真门控 & \tl{identity\_sim} & \tl{v\_frame(4)} \\
\dc{V-C2} & 场景道具一致 & \axC{} & 场景一致阈值锚 + 道具嵌入或比对跨镜 & \tl{scene\_consistency} & \tl{v\_frame(4)} \\
\dc{V-C3} & 风格一致 & \axC{} & CSD 风格嵌入逐帧与跨镜一致 + 检画风突变 & \tl{style\_csd} & \tl{v\_frame(4)} \\
\dc{V-C4} & 动作一致 & \axC{} & 动作识别与姿态跨镜比对 + 判动作连贯 & \tl{body\_structure} & \tl{v\_frame(4)} \\
\dc{V-C5} & 人景融合度 & \axC{} & ACP-Var~\citep{muss} / CPR + 判人景光影与透视融合，与 V-C1 对抗 & \tl{copypaste\_var} & \tl{v\_frame(4)} \\
\dc{V-C6} & 文字稳定 & \axC{} & 文字区逐帧 OCR + 相邻帧编辑距离 & \tl{ocr\_track} & \tl{v\_text(5)} \\
\dc{V-D1} & 运动平滑 & \axP{} & 光流帧间一致，抖动越低越平滑 & \tl{quality\_metric} & \tl{v\_frame(4)} \\
\dc{V-D2} & 动态幅度\,\fail{（已弃用）} & \axP{} & 光流幅度 + 镜头切换密度 & \tl{quality\_metric} & \textcolor{rulegray}{---} \\
\dc{V-D3} & 物理规律遵循 & \axP{} & VideoPhy-AutoEval 判物理常识，再结合画面判物理合理性 & \tl{videophy} & \tl{v\_frame(4)} \\
\dc{V-D4} & 因果时序合理性 & \axP{} & 子 agent 按时间窗描述 → 主 agent 判因果先后与动作完成 & \textcolor{rulegray}{---} & \tl{v\_frame(4)} \\
\dc{V-E1} & 语音质量 & \axE{} & DNSMOS 音质 + ASR 得 WER / CER 核台词 + 声纹相似度核音色 & \tl{dialogue\_align} \tl{asr\_wer} & \tl{v\_speech(7)} \\
\dc{V-E2} & 声画同步 & \axE{} & SyncNet 唇音同步 + ImageBind 音画对齐 & \tl{syncnet} \tl{imagebind\_av} & \tl{v\_sync(5)} \\
\dc{V-E3} & 音效与配乐 & \axE{} & 判配乐与音效同场景情绪、画面动作的贴合度 & \textcolor{rulegray}{---} & \tl{v\_audio(4)} \\
\dc{V-F1} & 构图 & \axE{} & 判景别 / 纵深 / 站位 + 主体框检测判砍头 & \tl{framing\_check} & \textcolor{rulegray}{---} \\
\dc{V-F2} & 运镜合理性 & \axE{} & 判运镜叙事意图、机位情绪与动能自然度 + 切换密度 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\dc{V-F3} & 人物表演能力 & \axE{} & 判表情与表演自然度 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{5} 集分镜视频}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{MV-C1} & 角色跨镜一致 & \axC{} & 各镜代表帧与首现镜身份相似度 + gap-decay + 服装比对 & \tl{identity\_sim}\,\fail{（空转）} & \tl{v\_frame(4)} \\
\dc{MV-C2} & 场景道具跨镜一致 & \axC{} & 场景库跨镜嵌入一致 + 道具状态嵌入或比对 & \tl{scene\_consistency} & \tl{v\_frame(4)} \\
\dc{MV-C3} & 风格跨镜一致 & \axC{} & CSD 风格嵌入跨镜一致 + 检画风突变 & \tl{style\_csd} & \tl{v\_frame(4)} \\
\dc{MV-C4} & 动作跨镜衔接 & \axC{} & 动作识别与姿态跨镜比对 + 输出朝向位置估机位判越轴 & \tl{axis\_check} \tl{body\_structure} & \tl{v\_frame(4)} \\
\dc{MV-C5} & 人景融合度 & \axC{} & 跨镜构图相似度过高告警 + 判人景融合，与 MV-C1 对抗 & \tl{framing\_check} \tl{copypaste\_var} & \tl{v\_frame(4)} \\
\dc{MV-C6} & 文字跨镜稳定 & \axC{} & 各镜文字区 OCR，跨镜比对同一文字元素内容一致 & \tl{ocr\_track} & \tl{v\_text(5)} \\
\dc{MV-D4} & 因果时序跨镜合理性 & \axP{} & 子 agent 按镜序描述事件 → 主 agent 判跨镜因果与闭环 & \textcolor{rulegray}{---} & \tl{v\_frame(4)} \\
\dc{MV-E1} & 语音跨镜质量 & \axE{} & 声纹跨镜相似度 + 逐镜全局音画对齐聚合 + ASR 衔接核 & \tl{imagebind\_av} \tl{asr\_wer} & \tl{v\_speech(7)} \\
\dc{MV-E3} & 音效与配乐跨镜 & \axE{} & 判配乐与音效跨镜的连贯统一与风格一致 & \textcolor{rulegray}{---} & \tl{v\_audio(4)} \\
\dc{MV-F3} & 表演跨镜连贯 & \axE{} & 判各段表情与情绪强度，比对段间过渡 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{6} 短剧成片}

{\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.28}
\setlength{\LTpre}{2pt}\setlength{\LTpost}{10pt}
\begin{longtable}{@{}p{0.95cm} >{\raggedright\arraybackslash}p{2.4cm}
  >{\centering\arraybackslash}p{0.5cm}
  >{\raggedright\arraybackslash}p{\dimexpr\textwidth-8.7cm-10\tabcolsep\relax}
  >{\raggedright\arraybackslash}p{2.9cm} >{\raggedright\arraybackslash}p{1.95cm}@{}}
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endfirsthead
\toprule
\textbf{编号} & \textbf{叶子维度} & \textbf{轴} & \textbf{实现方式} & \textbf{路由取证} & \textbf{可自调用工具} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{O-A1} & 事件完成 & \axF{} & 据剧本拆解关键事件清单 → 对照成片逐事件核实完成率 & \textcolor{rulegray}{---} & \tl{v\_frame(4)} \\
\dc{O-B1} & 风格 & \axC{} & CSD 全片风格嵌入一致性，色调按场景分组 & \tl{style\_csd} & \tl{v\_frame(4)} \\
\dc{O-B2} & 跨集一致 & \axC{} & 角色与场景库锚点 + gap-decay & \tl{identity\_sim}\,\fail{（空转）} \tl{scene\_consistency} & \tl{v\_frame(4)} \\
\dc{O-B3} & 跨集演进 & \axC{} & 对照剧本节点判有动机演进还是随意变化 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\dc{O-C1} & 成片可看性 & \axE{} & 校准后的整片总分 & \textcolor{rulegray}{---} & \textcolor{rulegray}{---} \\
\dc{O-C2} & 节奏转场 & \axE{} & 与人剪分布差异 + 转场自然度；切点检测量化剪辑节奏 & \textcolor{rulegray}{---} & \tl{v\_cut(5)} \\
\end{longtable}}\addtocounter{table}{-1}

\subsection{归因标签词表}
\label{sec:tagvocab}

任何低于 $5$ 分的打分，无论来自标注员还是来自自动化判分器，都必须从该维度声明的词表里
至少选一个标签；两侧取自同一份词表，这正是「看到了什么」能够与「打了多少分」分开比较的原因
。$66$ 个维度共声明 $298$ 个标签位、取自 $253$ 个互不相同的标签，
语料中累计 $255{,}925$ 条人工归因。每个维度另有\emph{其他}一项，下表中略去；
无论选中哪个标签，都必须同时填写自由文本理由。

\subsection*{\textcircled{1} 分镜设计}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{S-A1} & 事件覆盖 & 关键事件遗漏 $\cdot$ 次要情节遗漏 $\cdot$ 动作/旁白遗漏 $\cdot$ 事件不连贯 $\cdot$ 杜撰多余情节 $\cdot$ 情节交代含糊 \\
\dc{S-A2} & 对白保真 & 关键对白遗漏 $\cdot$ 篡改台词 $\cdot$ 说话人弄错 $\cdot$ 情绪语气错位 \\
\dc{S-B1} & 描述可执行性 & 描述含糊有歧义 $\cdot$ 视角不清楚 $\cdot$ 站位空间不清 $\cdot$ 一镜串多动作 $\cdot$ 单镜信息太空 $\cdot$ 文字冗长废话多 $\cdot$ 空间调度不可行 $\cdot$ 调度太复杂 \\
\dc{S-B2} & 补充适度性 & 漏补关键信息 $\cdot$ 转场衔接漏补 $\cdot$ 乱加多余细节 $\cdot$ 乱编不合理内容 \\
\dc{S-C1} & 叙事流畅度 & 转场太突然 $\cdot$ 衔接生硬突兀 $\cdot$ 镜内顺序颠倒 $\cdot$ 独白画外音错位 $\cdot$ 单镜景别混写 $\cdot$ 伏笔泄底 $\cdot$ 叙事繁琐冗余 $\cdot$ 前后矛盾 \\
\dc{S-C2} & 拍摄节奏 & 一镜塞太多动作 $\cdot$ 镜头太碎 $\cdot$ 重点戏镜头不足 $\cdot$ 过场太拖沓 $\cdot$ 缺反应镜头 $\cdot$ 运镜手段单一 \\
\dc{S-C3} & 情绪表达 & 节奏平淡无张力 $\cdot$ 缺情绪外化设计 $\cdot$ 冲突铺排混乱 \\
\dc{S-C4} & 视听风格处理 & 风格与剧种不符 $\cdot$ 风格杂乱不统一 $\cdot$ 重点戏缺渲染 $\cdot$ 镜头语言用错 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{2} 单张分镜图}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{I-A1} & 技术质量 & 画面模糊不清 $\cdot$ 噪点明显 $\cdot$ 伪影色块 $\cdot$ 黑影重影 $\cdot$ 水印乱码 $\cdot$ 结构扭曲畸变 \\
\dc{I-A2} & 美学风格 & 美学与剧种不符 $\cdot$ 画面元素杂乱 $\cdot$ 构图失衡 $\cdot$ 色彩光影不协调 $\cdot$ 画风不统一混搭 $\cdot$ 廉价AI感 \\
\dc{I-B1} & 主体属性 & 主体缺失 $\cdot$ 主体特征错漏 $\cdot$ 主体颜色错 $\cdot$ 主体材质错 $\cdot$ 主体数量错 $\cdot$ 多出主体 $\cdot$ 主体位置方位错 $\cdot$ 左右镜像错 $\cdot$ 表情神态不符 \\
\dc{I-B2} & 动作交互 & 动作没做出 $\cdot$ 动作做错 $\cdot$ 左右动作镜像 $\cdot$ 交互对象错 $\cdot$ 姿态生硬 \\
\dc{I-B3} & 场景与空间布局 & 场景类型错 $\cdot$ 方位摆错 $\cdot$ 遮挡关系错 $\cdot$ 相对位置错 $\cdot$ 场景元素缺失 \\
\dc{I-B4} & 镜头与视觉风格 & 景别视角不符 $\cdot$ 构图不符 $\cdot$ 光影氛围不符 $\cdot$ 画风不符 \\
\dc{I-C1} & 人脸身份 & 五官不像 $\cdot$ 脸型不符 $\cdot$ 神态表情不符 $\cdot$ 丢失特征 $\cdot$ 身份漂移 $\cdot$ 人物崩坏 \\
\dc{I-C2} & 外观服饰 & 发型不符 $\cdot$ 发色不符 $\cdot$ 服装款式不符 $\cdot$ 服装颜色不符 $\cdot$ 配饰缺失或错 $\cdot$ 不合身份时代 \\
\dc{I-C3} & 关键元素保真 \fail{（已弃用）} & 道具画错成别物 $\cdot$ 道具形态不符 $\cdot$ 道具颜色不符 $\cdot$ 道具材质不符 $\cdot$ 道具数量不符 $\cdot$ 道具缺失 \\
\dc{I-D1} & 角色跨图 & 跨图长相不一 $\cdot$ 跨图服饰不一 $\cdot$ 跨图配饰不一 $\cdot$ 身份漂移 $\cdot$ 人物崩坏 \\
\dc{I-D2} & 人景融合度（非贴图） & 人像抠图/贴片感 $\cdot$ 人景光影不匹配 $\cdot$ 悬浮不接地 $\cdot$ 姿态/表情雷同不变 $\cdot$ 多图复制粘贴 \\
\dc{I-D3} & 场景及布局（有场景参考） & 空间结构变样 $\cdot$ 物体方位变化 $\cdot$ 光向不一致 $\cdot$ 道具摆位变化 \\
\dc{I-D4} & 轴线（片段内） & 人物左右对调 $\cdot$ 位置方位偏移 $\cdot$ 跨图位移过大 $\cdot$ 视线方向错乱 $\cdot$ 运动方向反转 \\
\dc{I-D5} & 风格一致性 & 跨图画风不一 $\cdot$ 同场景色调不一 $\cdot$ 动漫真人混杂 \\
\dc{I-E1} & 人体结构合理性 & 多指/少指畸形 $\cdot$ 肢体扭曲粘连 $\cdot$ 肢体穿模 $\cdot$ 肢体缺失 $\cdot$ 面部比例失调 $\cdot$ 姿态违背常理 $\cdot$ 姿态僵硬不自然 \\
\dc{I-E2} & 环境物理合理性 & 物体悬浮 $\cdot$ 穿模穿墙 $\cdot$ 透视比例失真 $\cdot$ 光影倒影矛盾 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{3} 集分镜图}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{MI-D1} & 角色跨镜一致 & 跨段长相不一 $\cdot$ 跨段服饰不一 $\cdot$ 跨段配饰不一 $\cdot$ 身份漂移 $\cdot$ 跨段换脸 \\
\dc{MI-D2} & 人景融合度（非贴图） & 人像抠图/贴片感 $\cdot$ 人景光影不匹配 $\cdot$ 多段画面雷同 $\cdot$ 构图姿态不变 \\
\dc{MI-D3} & 场景跨镜一致 & 场景布局变化 $\cdot$ 陈设变化 $\cdot$ 光线色调变化 $\cdot$ 场景切换混乱 \\
\dc{MI-D4} & 空间方位连贯 \fail{（已弃用）} & 越轴左右对调 $\cdot$ 视线方向错乱 $\cdot$ 运动方向反转 $\cdot$ 拍摄方向/机位突变 \\
\dc{MI-D5} & 风格跨镜一致 & 画风跳变换画种 $\cdot$ 同场景色调不一 $\cdot$ 同场景光线不一 $\cdot$ 质感不统一 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{4} 分镜视频}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{V-A1} & 画质与材质 & 画面模糊低清 $\cdot$ 噪点伪影 $\cdot$ 材质失真 $\cdot$ 人物蜡感塑料感 \\
\dc{V-A2} & 美学画风与动态质感 & 构图色彩差 $\cdot$ 画风与剧种不符 $\cdot$ 廉价AI感 $\cdot$ 动态廉价粗糙 \\
\dc{V-B1} & 主体属性准确度 & 主体缺失 $\cdot$ 样貌不符参考 $\cdot$ 主体颜色错 $\cdot$ 主体材质错 $\cdot$ 主体数量错 $\cdot$ 多出主体 \\
\dc{V-B2} & 镜头与视觉风格 & 景别视角不符 $\cdot$ 构图不符 $\cdot$ 运镜不符指令 $\cdot$ 光影氛围不符 $\cdot$ 画风不符 \\
\dc{V-B3} & 帧图遵循 & 偏离给定帧图 $\cdot$ 运动中漂离参考 \\
\dc{V-C1} & 角色外观一致 & 主体闪烁抖动 $\cdot$ 样貌轻微改变 $\cdot$ 人物崩坏换脸 $\cdot$ 服装变色 $\cdot$ 服装款式变化 \\
\dc{V-C2} & 场景道具一致 & 背景布局变化 $\cdot$ 陈设变化 $\cdot$ 色调变化 $\cdot$ 道具状态突变 \\
\dc{V-C3} & 风格一致 & 画风突变 $\cdot$ 色调跳变 \\
\dc{V-C4} & 动作一致 & 动作衔接跳变 $\cdot$ 动作衔接生硬 $\cdot$ 动作前后矛盾 \\
\dc{V-C5} & 人景融合度（非贴图） & 人像抠图/贴片感 $\cdot$ 人景光影不匹配 $\cdot$ 悬浮不接地 $\cdot$ 姿态雷同不动 $\cdot$ 多帧复制 \\
\dc{V-C6} & 文字稳定 & 文字乱码 $\cdot$ 文字形变 $\cdot$ 文字闪烁 \\
\dc{V-D1} & 运动平滑 & 卡顿跳帧 $\cdot$ 瞬移 $\cdot$ 抖动 \\
\dc{V-D2} & 动态幅度 \fail{（已弃用）} & 画面过于呆滞 $\cdot$ 动作幅度失真 \\
\dc{V-D3} & 物理规律遵循 & 失重漂浮 $\cdot$ 穿模 $\cdot$ 碰撞不真实 $\cdot$ 惯性不自然 $\cdot$ 凭空出现消失 \\
\dc{V-D4} & 因果时序合理性 & 结果先于原因 $\cdot$ 事件时序颠倒 $\cdot$ 因果对不上 $\cdot$ 动作没做出 $\cdot$ 动作做错/不到位 \\
\dc{V-E1} & 语音质量 & 电音机械感 $\cdot$ 噪声破音 $\cdot$ 声音发闷模糊 $\cdot$ 音量不稳 $\cdot$ 台词念错漏字 $\cdot$ 台词乱序倒错 $\cdot$ 说话人对不上 $\cdot$ 含糊听不清 $\cdot$ 音色漂移换音 \\
\dc{V-E2} & 声画同步 & 唇音不同步 $\cdot$ 嘴动没声 $\cdot$ 声效错位 \\
\dc{V-E3} & 音效与配乐 & 配乐缺失 $\cdot$ 配乐不贴情绪 $\cdot$ 音效缺失 $\cdot$ 音效不贴画面 \\
\dc{V-F1} & 构图 & 景别失当 $\cdot$ 主体不突出 $\cdot$ 画面平板无纵深 $\cdot$ 主次混乱 \\
\dc{V-F2} & 运镜合理性 & 几乎无运镜 $\cdot$ 运镜乱飘无意图 $\cdot$ 运镜花哨多余 \\
\dc{V-F3} & 人物表演能力 & 表情呆滞单调 $\cdot$ 眼神朝向错 $\cdot$ 表演浮夸脱戏 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{5} 集分镜视频}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{MV-C1} & 角色跨镜一致 & 跨段长相不一 $\cdot$ 人物崩坏换脸 $\cdot$ 服装变色 $\cdot$ 服装款式变化 $\cdot$ 身份漂移 \\
\dc{MV-C2} & 场景道具跨镜一致 & 背景布局变化 $\cdot$ 陈设变化 $\cdot$ 色调变化 $\cdot$ 道具状态突变 \\
\dc{MV-C3} & 风格跨镜一致 & 画风突变换画种 $\cdot$ 同场景色调不一 $\cdot$ 动漫真人混杂 \\
\dc{MV-C4} & 动作跨镜衔接 & 动作衔接断层 $\cdot$ 动作前后矛盾 $\cdot$ 越轴左右对调 $\cdot$ 视线方向错乱 $\cdot$ 运动方向反转 $\cdot$ 拍摄方向/机位突变 \\
\dc{MV-C5} & 人景融合度（非贴图） & 人像抠图/贴片感 $\cdot$ 人景光影不匹配 $\cdot$ 多段画面雷同 $\cdot$ 机位构图不变 \\
\dc{MV-C6} & 文字跨镜稳定 & 跨段文字改变 $\cdot$ 文字乱码 $\cdot$ 文字形变 \\
\dc{MV-D4} & 因果时序跨镜合理性 & 跨段结果先于原因 $\cdot$ 跨段事件时序颠倒 $\cdot$ 跨段因果对不上 $\cdot$ 动作跨段没收尾 \\
\dc{MV-E1} & 语音跨镜质量 & 跨段音色漂移换音 $\cdot$ 跨段音量不稳 $\cdot$ 跨段音质不一 $\cdot$ 台词跨段断裂 \\
\dc{MV-E3} & 音效与配乐跨镜 & 配乐跨段断片 $\cdot$ 配乐切换突兀 $\cdot$ 音乐风格跳变 $\cdot$ 音效跨段不一 \\
\dc{MV-F3} & 表演跨镜连贯 & 段间情绪断裂 $\cdot$ 情绪强度跳变 $\cdot$ 表演风格忽变 $\cdot$ 跨段表演脱戏 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection*{\textcircled{6} 短剧成片}

{\scriptsize
\setlength{\LTpre}{2pt}\setlength{\LTpost}{8pt}
\begin{longtable}{@{}p{1.05cm} >{\raggedright\arraybackslash}p{3.7cm} >{\raggedright\arraybackslash}p{\dimexpr\textwidth-4.75cm-4\tabcolsep\relax}@{}}
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endfirsthead
\toprule
\textbf{编码} & \textbf{维度} & \textbf{归因标签} \\
\midrule
\endhead
\bottomrule
\endlastfoot
\dc{O-A1} & 事件完成 & 关键事件缺失 $\cdot$ 事件未演完 $\cdot$ 主线断裂 $\cdot$ 人物指认错乱 $\cdot$ 杜撰偏离剧本 \\
\dc{O-B1} & 风格 & 集间风格断层 $\cdot$ 同场景色调不一 $\cdot$ 画风不统一 \\
\dc{O-B2} & 跨集一致 & 角色跨集变样 $\cdot$ 标志特征不一 $\cdot$ 场景跨集变样 $\cdot$ 跨集换脸 \\
\dc{O-B3} & 跨集演进 & 角色未转变 $\cdot$ 服装未转变 $\cdot$ 外观场景乱改 $\cdot$ 变化突兀无铺垫 \\
\dc{O-C1} & 成片可看性 & 成片不完整 $\cdot$ 廉价感强 $\cdot$ 硬伤多看不下去 \\
\dc{O-C2} & 节奏转场 & 重点戏一带而过 $\cdot$ 过场拖沓 $\cdot$ 节奏忽快忽慢 $\cdot$ 转场生硬 \\
\end{longtable}}\addtocounter{table}{-1}

\subsection{判分 prompt}
\label{sec:prompt}

全部 $66$ 个维度共用一个 prompt 模板。所有与维度相关的内容都注入固定的槽位，
这正是判分可审计的原因：两个维度可以打分不同，但不可能框架不同。骨架如下，槽位已标出：

\begin{quote}\small\ttfamily\raggedright
你是短剧生成质量评测子 agent。请只对单个维度【\{编号\} \{名称\}】（评测轴 \{轴\}，标准化层 \{层\}）给出 5 档评分。\\[3pt]
【五档评分锚点】: \{五档判据 5..1\}\\
【逐镜检查要点与定档规则】: \{可选 · 逐条核查清单在此\}\\
【是否适用（先判 N/A 再打分）】: \{可选\}\\
【可选归因标签】(分数<5 时必须至少选一个): \{该维度标签表\}\\
【自动化方法提示】: \{method\}\\
【样本】stage=\{\dots\} scope=\{\dots\} paradigm=\{\dots\}\\
【原始剧本（对照基准 · ground truth，非被评内容）】: \{条件注入\}\\
【客观工具取证结果】: \{取证结果，每条度量一行\}\\
【打分硬性要求（对所有维度生效）】: \{常量\}\\
严格只输出 JSON: \{"score", "confidence", "tags", "reason"\}
\end{quote}

常量框架里有四段真正起作用，其中两段按运行原文引用。
一条反套路规则禁掉了会造出人为分布的那类措辞：
\zhq{严禁用『按评分压缩原则 / 保守起见 / 一般不给满分 / 整体不错但仍扣一分』等无实据、套路化或人为往中间档或极端档拉的措辞来给分。分数只由画面/证据里的真实缺陷决定，不做任何人为分布调整。}
一条严重程度校准让扣分与观感成正比而不是逐项累加：
\zhq{扣分幅度要匹配该缺陷对【整体观感】的实际影响……多个瑕疵时按对观感的综合影响定档，不要把每个小瑕疵逐一叠加扣分导致过低。}
另两段把分数与证据绑住：凡低于 $5$ 分必须指出具体、可核验的缺陷，
并从该维度词表中至少选一个归因标签；而在有核查清单的图阶段，
理由必须以逐条核查结论开头、逐条对应清单序号，不能用一句总结代替。

\paragraph{多轮循环。}
凡声明了可自调用工具的维度，打分是一个循环而不是一次调用。
第 $0$ 到 $n-1$ 轮把工具 schema 开放出来、由模型自己决定调不调；
每次工具结果追加进对话历史，裁切出来的图作为下一轮的媒体回喂。
最后一轮把工具整个撤掉，这才是逼出裁决的那一步。
同一个工具带同一组参数重复调用超过两次会返回一个错误；
若跑完所有轮次仍未给出合法 JSON，会再补一轮无工具的收尾，之后才回落到一次性判分。

\subsection{取证工具链}
\label{app:toolchain}

支撑上述两条路径的两套注册表，按家族列于 \cref{tab:tools}。

\begin{table}[htbp]
\centering
\caption{取证工具，按家族分：自动化评测可自行调用的那些，加上总是自动运行的路由度量。
名称为注册表标识符的简写。没有任何一个工具产出判据档位，尽管其中若干会给出自己的数值。}
\label{tab:tools}
\small
\begin{tabular}{@{}l p{11.2cm}@{}}
\toprule
\textbf{家族} & \textbf{工具} \\
\midrule
视觉   & \texttt{zoom\_in}（裁切放大）、\texttt{draw\_bbox}（标注区域）、
         \texttt{count\_marker}（编号点计数），
         以及对 \texttt{pixel\_sensitive} 维度不开放的三个改像素工具
         （\texttt{sharpen}、\texttt{super\_resolution}、\texttt{enhance\_contrast}）。
         宫格图在评一致性之前先切成子格。 \\
时序   & \texttt{extract\_frame}（按时间戳采帧，抽出的帧还可以再放大）、
         \texttt{detect\_scenes}（镜头切分）、\texttt{video\_probe}（容器元数据）。 \\
听觉   & \texttt{asr\_segment}（转写）、\texttt{dnsmos}（无参考音质）、
         \texttt{detect\_audio\_events}、\texttt{extract\_subtitles}（烤进画面的字幕轨）、
         \texttt{extract\_clip\_audio}、\texttt{ocr\_frame}。 \\
专项度量 & 属于路由而非模型自调：\texttt{videophy}（物理合理性）、
         \texttt{syncnet} $+$ \texttt{imagebind\_av}（声画同步）、\texttt{identity\_sim}（角色一致）、
         \texttt{copypaste\_var}（人景融合，反「贴图」）、\texttt{ocr\_track}（文字稳定）、
         \texttt{cut\_detect}（镜头切换，随基础上下文注入而不走路由），以及无参考画质模型；
         美学打分模型会算，但在每个环节都被扣下不进 prompt。其中若干会给出自己的数值；
         某个数值是否采信，仍按 \cref{sec:step2} 的相关性检验逐个过筛，且多数已被它取消锚点资格。 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{成本与可靠性。}
单题墙钟耗时中位 $14.6$ 分钟。工具是并发执行的，所以累计机时远大于这个数：
单维工具机时中位 $198.7$ 秒，单次作业中位 $20$ 次子 agent 调用、约 $19$ 次度量调用。
度量类路由覆盖 $21$ 个视频叶子维度中的 $17$ 个。
八个主要工具里只有 \texttt{ocr\_track} 的可用率掉到 $98.9\%$ 以下，为 $71.1\%$。
这些成本绝大部分花在工具执行而不是推理上，所以多轮推理几乎不增加成本，而增挂工具的成本很高。

\subsection{候选指标的验证}
\label{sec:audit}

每个候选指标都要拿人工共识来检验，而不是凭它「本来是为什么做的」就采信。
审计按粒度各做一次，每次只上该粒度适用的那批工具，
并与这批工具能对上的每一个人工维度做相关，用的是该粒度的全量标注语料，
SRCC 与 $p$ 分别在各生成范式内与混池两种口径下计算。
一个工具往往给出多个标量字段而不是一个（仅 \texttt{quality\_metric} 一个就返回
MUSIQ、TOPIQ-NR、拉普拉斯锐度、亮度与对比度），每个字段都单独检验。
一致性只决定一件事：这个数值能不能当判分锚点用。
一个小模型要不要留下来是另一件事，取决于它是否提供了判分模型光靠看拿不到的底层感知信号。

\paragraph{受检候选。}
\emph{结构与主体}：YOLO26n~\citep{yolo26} $+$ SAM2.1~\citep{sam2,sam21} 做计数与分割，
YOLO26n-pose~\citep{yolo26} 做人体结构、
构图与画面朝向。\emph{身份与一致}：ArcFace~\citep{arcface}、OSNet Re-ID~\citep{osnet}、
DINOv3 通用特征相似度~\citep{dinov3} 做角色，DreamSim~\citep{dreamsim} 做场景，
CSD ViT-L~\citep{csd} 做风格。\emph{画质与美学}：MUSIQ~\citep{musiq}、
TOPIQ-NR~\citep{topiq}、NIMA~\citep{nima}、DOVER 与 DOVER++~\citep{dover}、拉普拉斯锐度、
RAFT~\citep{raft} 光流。\emph{声音}：Whisper~\citep{whisper} ASR（faster-whisper）、
DNSMOS~\citep{dnsmos}、GE2E~\citep{ge2e} 声纹（Resemblyzer）、SyncNet~\citep{syncnet} 唇音同步、
ImageBind~\citep{imagebind} 音画语义对齐。\emph{大模型旁证}：
Q-Judger~\citep{qwenimagebench}、ArtiMuse~\citep{artimuse}、
UniPercept~\citep{unipercept}、VideoPhy-AutoEval~\citep{videophy2}。

\paragraph{结果。}
按我们为「够格当判分锚点」设的标准（至少 $100$ 题上 $|\mathrm{SRCC}| \ge 0.3$），
大多数候选都达不到这条线，而且失效不止一类：结构与主体、身份与一致、画质与美学、
以及 AIGC 专用判别都在其中。八个代表性数值可以看出量级：
通用组这一侧，NIMA 美学为 $-0.152$、拉普拉斯锐度 $-0.144$、TOPIQ-NR $-0.067$、MUSIQ $-0.057$；
AIGC 专用这一侧，Q-Judger 为 $0.004$、ArtiMuse $0.030$，
UniPercept 的画质头为 $0.190$、美学头为 $0.110$。

\paragraph{两侧为何都够不到。}
在 AI 短剧里，画质的判断标准看起来是依附于题材与美术风格的，而不是画面自身的一项属性。
玄幻爽剧会主动拉高饱和度来强化商业观感，而在另一些题面里同样夸张的色彩正是 AI 感最明显的破绽。
同一视觉特征因此不能作为统一判据，这也是两组模型出现系统性误判最合理的来源：
通用组标定在自然照片上，AIGC 专用组回答的是「这张图好不好看」，
而不是「这一格有没有按剧本做对」。

\paragraph{我们怎么用它们。}
与其不加验证就把这些指标挂上去，我们把小模型留作底层证据的来源，不让它们直接输出分数。
凡数值要呈给判分模型的，只给实测值与一条方向说明，不给标定过的参考档位；
例外是物理、参照相似度与声纹这几组字段，它们仍保留档位。
美学打分模型是唯一算了却从不呈给模型的候选：它在每个环节都在进 prompt 之前被丢掉。
屏蔽是分环节的而不是全局的：以 DOVER 为例，它在视频阶段是弱\emph{正}相关，
若在那里也一并屏蔽，会连一个符号正确的信号一起删掉。

\subsection{基于人工标注的训练}
\label{app:train}

训练遵循 \cref{sec:judgetrain} 中的 SFT--GRPO 流程。每个训练样本是针对一道题、一条评测轴与一种输出形式的提示，
分数与归因的监督都来自人工标注。输出保留 \judger{} 按轴组织的结构，包括叶子维度分数、简短理由与综合分。
\cref{sec:ablation} 中的测试题在两个训练阶段中都被排除。

分镜图与分镜脚本判分模型不使用音频通路。归因奖励使用每道题已有的人工标注；缺失的标注不计为失败。
分镜脚本的训练不使用归因奖励。

采用贪心解码时，每个「题目--评测轴--输出形式」提示的推理耗时，不输出推理时为 $6$--$9$\,秒，输出推理时为 $13$--$27$\,秒。
这些耗时针对单个提示，而不是对全部适用评测轴的完整评测，
因此与 \judger{} 逐题的墙钟耗时（\cref{app:toolchain}）分开报告。


==> sections_zh/B_dramas.tex <==
\section{剧目清单}
\label{app:dramas}

剧本语料共 $20$ 部剧、每部 $10$ 集，覆盖不同受众频道、年代主题与题材；
其中真人 $10$ 部、动画 $10$ 部，台词中文 $16$ 部、英文 $4$ 部，使每个切面都够做分层核查（\cref{sec:slices}）。
各环节均取每部剧的前 $3$ 集，共 $60$ 集。\pipe{} 基于这些剧本生成分镜、分镜图、分镜视频与成片。
逐部清单见 \cref{tab:dramas}。

每部剧有统一的角色名册，分集大纲每集三百到五百字。
剧本遵循红果拍摄稿格式规范，含场号、地点与时段、人物表、动作行、镜头标注与带情绪提示的台词。

\begin{table}[htbp]
\centering
\caption{剧目清单。英文档为 $2$ 真人 $+$ $2$ 动画，场景描述一律中文，
差别只在台词与屏幕文字，这正是把语言效应与生产难度分离开的做法。}
\label{tab:dramas}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.18}
\begin{tabularx}{\linewidth}{@{}l l >{\raggedright\arraybackslash}X c c r@{}}
\toprule
\textbf{频道} & \textbf{年代 / 主题} & \textbf{题材 / 剧名} &
\textbf{语言} & \textbf{画风} & \textbf{集} \\
\midrule
\multirow{7}{*}{男频} & 都市现代 & 战神归来 ——《归刃》 & 中文 & 动画 & 3 \\
 & 都市现代 & 赘婿逆袭 ——《赘婿无锋》 & 中文 & 真人 & 3 \\
 & 都市现代 & 神豪炫富 ——《散财令》 & 中文 & 真人 & 3 \\
 & 古装历史 & 权谋朝堂 ——《沉冤录》 & 中文 & 真人 & 3 \\
 & 古装历史 & 穿越逆袭 ——《明朝火锅记》 & 中文 & 动画 & 3 \\
 & 奇幻脑洞 & 末日求生 ——《冻土堡垒》 & 中文 & 动画 & 3 \\
 & 奇幻脑洞 & 重生逆袭 ——《重来不渡》 & 中文 & 真人 & 3 \\
\addlinespace[2pt]
\multirow{3}{*}{全性向} & 奇幻脑洞 & 穿越异世 ——《白垩开荒》 & 中文 & 动画 & 3 \\
 & 近代现代 & 青春校园 ——《那年蝉鸣》 & 中文 & 真人 & 3 \\
 & 近代现代 & 乡村种田 ——《麦囤满仓》 & 中文 & 动画 & 3 \\
\addlinespace[2pt]
\multirow{6}{*}{女频} & 都市言情 & 先婚后爱 ——《偏偏暖你》 & 中文 & 真人 & 3 \\
 & 都市言情 & 真假千金 ——《不稀罕》 & 中文 & 动画 & 3 \\
 & 都市言情 & 豪门虐恋 ——《替月》 & 中文 & 动画 & 3 \\
 & 古代言情 & 古装穿越 ——《躺赢娘娘》 & 中文 & 真人 & 3 \\
 & 古代言情 & 强取豪夺 ——《偏要抢卿》 & 中文 & 动画 & 3 \\
 & 大女主无 CP & 女性成长 ——《翻山》 & 中文 & 真人 & 3 \\
\addlinespace[2pt]
\multirow{2}{*}{海外男频} & 都市现代 & 逆袭复仇 —— \emph{The Janitor's Billion-Dollar Revenge} & 英文 & 动画 & 3 \\
 & 都市现代 & 隐藏富豪 —— \emph{The Bellboy Owns This Hotel} & 英文 & 真人 & 3 \\
\addlinespace[2pt]
\multirow{2}{*}{海外女频} & 都市现代 & 血族之恋 —— \emph{The Vampire Lord's Forbidden Blood} & 英文 & 动画 & 3 \\
 & 都市现代 & 契约婚姻 —— \emph{The Billionaire's Two-Year Wife} & 英文 & 真人 & 3 \\
\midrule
\multicolumn{5}{@{}l}{\textbf{合计}} & \textbf{60} \\
\bottomrule
\end{tabularx}
\end{table}

\input{figures/fig_exhibit}


==> sections_zh/H2_agreement.tex <==
\section{自动化评测的一致性切面}
\label{app:agreeslices}

下面四个切面把语料固定住，改变的是判分对象：环节、评测轴、模态，
以及人的判断在这条维度上有多可复现（\cref{tab:agreeslices}）。四者问的是同一个问题：
自动化评测在哪里仍然与三人共识吻合。所有数值都是对三人共识的逐题一致性，
或直接给出，或以留一法人工基线的倍数给出。
两侧榜单都是连续的均分而不是类别标签，因此一致性以相关系数报告；
\cref{app:slices} 中的效应也按分数单位给出而不做标准化~\citep{cohend}，这样才能与 $3.0$ 可用线直接比较。

\begin{table}[htbp]
\centering
\caption{四个一致性切面：各自改变什么，以及一致性在哪里不再成立。}
\label{tab:agreeslices}
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}l l l@{}}
\toprule
\textbf{切面} & \textbf{改变什么} & \textbf{一致性在哪里不再成立} \\
\midrule
链路环节 & 六个粒度 & 在图与视频之间跨过人工基线 \\
评测轴   & 五条评测轴 & 沿可核查 $\rightarrow$ 感知 $\rightarrow$ 审美递减 \\
模态 & 文本、像素、时序与音轨 & 同一条判据在三者上逐级失效 \\
人工共识水平 & 人的判断有多可复现 & 自动化评测准的恰好是人也能达成共识的那些维度 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\subsection{按环节：在图与视频之间跨过人工基线}
\label{sec:slice-stage}

以留一法人工基线的倍数来读，逐题一致性在分镜设计上是 $2.35$ 倍、单分镜图 $1.19$ 倍、
集分镜图 $1.48$ 倍，到三档视频则依次为 $0.79$、$0.85$、$0.85$ 倍（\cref{tab:agree}）。
也就是说图像这一侧落在 $1.19$--$2.35$ 倍，视频这一侧落在 $0.79$--$0.85$ 倍，
而跨过 $1$ 倍的位置在图像与视频环节之间，不在单条与多条素材之间：
集分镜图已经要求跨镜比对，却仍在基线之上；单条 clip 只判一个孤立产物，却已经在基线之下。
起决定作用的是被判对象的模态，而不是它在链路上的深度（\cref{fig:ratio}）。

\subsection{按评测轴：判据越缺外部参照，一致性越低}
\label{sec:slice-axis}

把 $63$ 个叶子维度归并到五条轴上，逐题一致性依次为 \axF{} $0.423$、\axC{} $0.235$、
\axP{} $0.146$、\axE{} $0.132$、\axQ{} $0.121$（\cref{tab:axes}）。
只有 \axF{} 相对人工基线取得净提升（$+0.107$，$12$ 维中 $9$ 维占优）；
\axQ{} 的四维一个都没有超过基线，整体低出 $0.086$。
这个次序跟的是判据能在产物之外核对到多少东西（\axF{} 可以核对上游产物，
\axC{} 可以核对同批产物，\axQ{} 什么都没有），
这也正是那批小模型画质指标无一够格当判分锚点的同一条分界（\cref{sec:audit}）。
这一层是把三种模态混在一起算的，同一条轴换到不同模态上还会再分化。

\subsection{按模态：同一条判据从文本到像素到时序逐级失效}
\label{sec:slice-axismod}

\cref{tab:axes} 是把模态压掉之后的逐轴分解，\cref{tab:axismod} 则保留两个因子，在 \cref{sec:modality} 中解读。
最清楚的一例是 \axE{}：在分镜脚本的文本模态下，它高出人工基线 $0.175$，$4$ 维全胜；
同一条判据落到带时序与音轨的视频上，则低于基线 $0.190$，$11$ 维全败。
\axF{} 在同样三种模态上单调衰减（文本 $+0.317$、像素 $+0.101$、时序与音轨 $+0.012$），
而 \axQ{} 在它有定义的两种模态上都低于基线。
因此一条轴在某个模态上通过了校验，不能假定它在下一个模态上同样成立，
这也是本报告不给出脱离模态的单一一致性数值的原因。

\input{figures/tab_axes}

\subsection{按人工共识：人能达成共识处才判得准}
\label{sec:slice-consensus}

最后一个切面换掉的是自变量：不看评的是什么内容，只看这条维度上人的判断有多可复现。
在 $63$ 个叶子维度上，人工基线与自动化评测的相关是 PLCC $0.418$（SRCC $0.416$）：
人工一致性较高的维度，自动化一致性往往也较高，两者并非各有所长（\cref{fig:scatter63}）；
这种关联并不说明任何一方的评分是准确的。
由此有两点：两侧都低的地方，症结在判据本身的可操作性，而不在标注预算或提示词工程，
在那里继续调优自动化方法收益很低；以及决定弃用一个维度时，
该看的是人工基线而不是自动化分数。标注员自己都无法复现的维度，
自动化评测没有可对齐的目标。

\input{figures/fig_scatter63}


==> sections_zh/H_slices.tex <==
\section{自动化分数的内容切面}
\label{app:slices}
\label{sec:slices}

本附录的三个切面改变的是生成对象：剧的画风、台词语言，以及链路交给模型的输入范式
（\cref{tab:slices}）。它们考察的是自动化绝对分随之移动的幅度（\cref{tab:slicefx}）。
三种效应的大小次序是：输入范式最大，画风次之，台词语言最小。

\begin{table}[htbp]
\centering
\caption{三个内容切面：各自改变什么，以及对自动化分数做了什么。}
\label{tab:slices}
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}l l l@{}}
\toprule
\textbf{切面} & \textbf{改变什么} & \textbf{对自动化分数的影响} \\
\midrule
画风     & 真人对动画 & 五个粒度上偏向真人 $0.08$--$0.22$ 分 \\
台词语言 & 英文对中文台词 & 最多 $0.12$ 分，且几乎全部落在 \axF{} 上 \\
输入范式 & 首尾帧、宫格、多参考 & 最大 $0.42$ 分，且在两档分镜图之间反向 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\input{figures/tab_slicefx}

\subsection{按画风：真人档分更高}\label{sec:slice-style}

在跑了两种画风的模型内部，自动化综合分在六个粒度里有五个偏向真人档，幅度 $0.08$--$0.22$ 分；
唯一的例外是单分镜图，反向 $0.08$ 分（\cref{tab:slicefx}）。
综合分把机制藏起来了，因为有两条轴方向相反：分镜视频上 \axC{} 在真人档高 $0.32$，
\axQ{} 在动画档高 $0.25$，而 \axF{} 两侧相同。
逐维的极值更大，\dc{V-C3} 风格一致偏向真人超过一整分，\dc{V-A1} 画质与材质则偏向动画约三分之二分。
换画风换掉的是会被找出来的缺陷类型，而不是让题目整体变容易。

\subsection{按台词语言：效应很小，只落在保真轴上}\label{sec:slice-lang}

场景描述一律中文，所以四部英文台词剧与其余十六部只在台词与屏幕文字上不同，
两档在画风上也是配平的。自动化综合分在每个粒度上都偏向英文，但从未超过 $0.12$ 分
（\cref{tab:slicefx}），而这点移动几乎全部落在一条轴上：\axF{} 在短剧成片上英文高 $0.64$，
而 \axQ{} 在它有定义的两个粒度上两位小数完全相同。
移动的都是承载语言的维度（事件完成、语音质量、对白保真），
反向的则是角色跨镜一致与跨集一致。
语言移动的是承载语言的那些维度，而不是承载像素的那些维度。

\subsection{按输入范式：最大，且沿链路反向}\label{sec:slice-para}

输入范式平均而言是三者中影响最大的一个，也是唯一一个方向沿链路不稳定的：
单分镜图上首尾帧领先宫格 $0.37$ 分，集分镜图上却落后 $0.42$ 分，而三档视频上宫格都居首，
只是在分镜视频与短剧成片上领先得很小（\cref{tab:slicefx}）。
单分镜图这一比要先做一处修正，因为整条 \axC{} 轴在那里只在宫格下存在，
限制到共有的十个维度后，首尾帧的领先\emph{扩大}到 $0.61$。
每种范式的强项，往往落在它的输入所固定的那部分上。首尾帧交出两端帧图，
于是在分镜图环节领先 \axF{} 输入保真（$3.57$ 对 $2.73$），
在分镜视频上领先以给定帧为锚的场景道具一致与镜头风格，却在运镜合理性上落后，
因为两端把镜头运动约束得过死；宫格用一张图承载整集，
于是领先跨镜一致（集分镜图 $3.53$ 对 $3.11$）与构图，代价落在声画同步；
多参考没有可遵循的帧图，于是 \axF{} 垫底（$2.92$ 对 $3.39$），
而在没有别的东西去约束的运镜合理性、声画同步与 \axE{} 影视表现力上最好。


==> sections_zh/I_cases.tex <==
\section{案例分析}
\label{app:cases}

下面的案例依次说明：一个分数藏起了什么（\cref{app:pairs}、\cref{app:crossshot}）、被藏起来的缺陷从哪里来
（\cref{app:shotcase}--\labelcref{sec:degrade}）、把分数拆开后各模型有何不同（\cref{app:profiles}、\cref{app:seedance}），
以及自动化评分在哪里失手（\cref{app:judgefail}）。

\FloatBarrier
\subsection{分数相近，缺陷形态不同}
\label{app:pairs}

\input{figures/qual_boxed_image}

\cref{fig:qual:boxed} 是强制归因的论据。四道题都在某个维度上的三人均分为 $1.3$--$1.7$ 分，
综合分会把它们排在一起，而标注框落在四个互不相交的位置：脸上、动作中的肢体上、
本不该在场的人物上、手指数目错误的手上。每一对里两个模型还互换了失败的维度：
丢身份的那个把动作保住在 $3.0$，丢动作的那个把身份保住在 $3.33$。
这是 \cref{sec:closepairs} 的逐题版本。

\FloatBarrier
\subsection{跨镜一致是一项独立能力}
\label{app:crossshot}

\input{figures/qual_crossshot}

\cref{fig:qual:crossshot} 直接说明了这一点。两个模型画同一集、用同一套设定卡，
榜首档那一行的两位主角跨镜稳住了，末档那一行没有：\dc{MI-D1} 的三人均分相差 $2.66$ 分。
真正重要的性质是\emph{失败那一行里的每一张单独看都无可指摘}：镜 $7$ 单看没有任何错，
它错在与镜 $5$ 的关系上。单条榜不是在低报跨镜质量，它测的是另一个量。

\FloatBarrier
\subsection{镜头数与分镜可执行性}
\label{app:shotcase}

\cref{tab:shots3612} 把三个模型放在同一份分集剧本上，且只在分镜环节分叉。
三镜那份产物把整集压进三个镜头，自标时长合计 $30$\,秒、对白 $10$ 段；
三名标注员都把它的描述可执行性（\dc{S-B1}）与拍摄节奏（\dc{S-C2}）打到 $1.00$、分歧度 $0.00$，
标出的缺陷每次都是同样几类：一镜多动作、走位复杂到不可执行、缺反应镜头。
加到六个镜头，两个 \axF{} 维度直接回满；再加到十二个，只换来描述可执行性的提升
（\cref{fig:shotcount}）。

\begin{table}[htbp]
\centering
\caption{同一份分集剧本、三个模型、三种镜头数。分数为三名标注员评分的均值。
只有分镜环节分叉，三个模型收到的是同一份剧本。}
\label{tab:shots3612}
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}l l r r r l@{}}
\toprule
\textbf{叶子维度} & \textbf{轴} &
\makecell{\md{mimo-v2.5-pro}\\\footnotesize 3 镜} &
\makecell{\md{gpt-5.5-xhigh}\\\footnotesize 6 镜} &
\makecell{\md{claude-opus-4.8-max}\\\footnotesize 12 镜} &
\textbf{行为} \\
\midrule
\dc{S-A2} 对白保真 & \axF & \fail{1.33} & \best{5.00} & \best{5.00} & 到 6 镜就不再漏台词 \\
\dc{S-A1} 事件覆盖 & \axF & \fail{2.67} & \best{4.67} & \best{4.67} & 同上 \\
\dc{S-B1} 描述可执行性 & \axP & \fail{1.00} & 3.00 & \best{4.00} & 随镜头数单调上升 \\
\dc{S-C2} 拍摄节奏 & \axE & \fail{1.00} & \best{3.67} & \best{3.67} & 6 镜已经够 \\
\addlinespace[2pt]
整体印象 & & \fail{1.67} & \best{4.00} & \best{4.00} & --- \\
\addlinespace[2pt]
标出的问题数 & & 23 & 18 & 15 & 变少，且性质在变 \\
三人分歧度 & & 1.75 & 0.75 & 0.63 & 产物越差越难打分 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

\input{figures/fig_shotcount}

\FloatBarrier
\subsection{不同输入范式暴露不同的失效形态}
\label{app:paradigmcase}

\input{figures/qual_paradigm_disease}

\cref{fig:qual:disease} 把两种特征失效形态并列，而两种失败对另一种范式都不可能发生：
宫格漏画人物，因为一张图要填满多个格子；首尾帧在两张帧图之间换人，
因为首尾两帧不是一次生成的，身份在两次生成之间没有被保持住。
这正是难度由范式而非画风决定的原因，也是混池会稀释宫格塌陷的原因。

在视频侧，同一条分界逐题可见（\cref{tab:paradigm}）。宫格范式下 \md{pixverse-c1} 的某一镜
在帧图遵循上的三人均分为 $1.67$ 分，三名标注员标出的缺陷全部只有一类：「偏离给定帧图」，
分别定位在 $0.29$--$11.04$\,s、$2.98$--$4.87$\,s 与 $6.56$--$8.15$\,s。
这个范式下的提示词只描述运镜与对白，角色造型与走位就只由那张宫格图锚定。
一旦宫格被拆成子格再当输入，对它的遵循度就明显弱于对首尾帧对的遵循度。

\FloatBarrier
\subsection{上游缺陷延续到下游}
\label{sec:degrade}

\input{figures/qual_drift}

\cref{fig:prop} 使用四部剧（两真人、两动画），全程首尾帧范式，视频模型固定。
基线链路在三个粒度上的自动化得分均最高（$3.03$--$3.29$）；四种替换各换掉一个上游环节，
并在三个粒度上读取（\cref{sec:prop}），
这些链路由自动化评测打分，没有人工标注。
\cref{fig:qual:drift} 在单题上展示了上游一侧：陈设在连续关键帧之间发生变化，而人物身份保持稳定。

\subsection{\texorpdfstring{\md{hy4-preview}}{hy4-preview} 与 \texorpdfstring{\md{hy3}}{hy3}：保真与制作可执行性}
\label{app:profiles}

\cref{tab:hy3} 展开了 \cref{tab:main} 中的自动化分镜比较。
\md{hy4-preview} 的综合分高于 \md{hy3}（$4.02$ 对 $3.89$），\axF{}（$4.69$ 对 $4.36$）与 \axE{}（$3.91$ 对 $3.78$）更高，
但 \axP{} 更低（$3.56$ 对 $3.65$）。更好地还原剧本，并不意味着更好的制作可执行性。
\md{hy3} 与 \md{doubao-seed-2.1-pro} 的综合分同为 $3.89$，但后者在情绪表达与叙事流畅上领先。

\begin{table}[htbp]
\centering
\caption{分镜自动化均分（按列顺序 $n=60/57/60$）。样本并非完全配对；\md{hy4-preview} 只有自动化评分。}
\label{tab:hy3}
\small
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{@{}l l r r r@{}}
\toprule
\textbf{叶子维度} & \textbf{轴} & \md{hy4-preview} & \md{hy3} & \md{doubao-seed-2.1-pro} \\
\midrule
\dc{S-A1} 事件覆盖 & \axF & \best{4.53} & 4.31 & 4.27 \\
\dc{S-A2} 对白保真 & \axF & \best{4.84} & 4.42 & 4.25 \\
\dc{S-B1} 描述可执行性 & \axP & 3.73 & 3.82 & \best{3.90} \\
\dc{S-B2} 补充适度性 & \axP & 3.38 & \best{3.48} & 3.40 \\
\dc{S-C1} 叙事流畅 & \axE & 4.33 & 4.26 & \best{4.40} \\
\dc{S-C2} 拍摄节奏 & \axE & \best{3.05} & 2.91 & 2.58 \\
\dc{S-C3} 情绪表达 & \axE & 4.23 & 4.05 & \best{4.33} \\
\dc{S-C4} 视听风格 & \axE & \best{4.03} & 3.89 & 3.99 \\
\addlinespace[2pt]
综合 &  & \best{4.02} & 3.89 & 3.89 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\tabnote{加粗为每行最高均值；综合为八个叶子维度的均值。}
\end{table}

在动画剧《偏要抢卿》第 $2$ 集（$20$ 段对白）上，三份产物分别以 $10/10/7$ 个镜头逐字保留了 $20/20/3$ 段对白：
\md{hy4-preview} 补充了运镜与走位，但会在一个镜头里串联多个动作；\md{hy3} 除「快切」「特写」外补充很少；
\md{doubao-seed-2.1-pro} 补充了画面细节，却改写了对白。

从人工一侧看，按有人工标注的分镜题上三名标注员的均分，\md{hy3} 的综合分为 $3.43$（$57$ 题），
\md{doubao-seed-2.1-pro} 为 $3.60$（$60$ 题）。在八个叶子维度上，\md{hy3} 名次最高的是对白保真
（$4.44$，九个模型中第 $4$，落后该维榜首 $0.20$ 分），名次最低的是情绪表达（$3.64$）与视听风格处理（$3.91$），
同为九个模型中第 $8$。在上面比较的那一集里，三名标注员都把 \md{doubao-seed-2.1-pro} 的对白标为篡改或漏字。

\subsection{\texorpdfstring{\md{seedance-2.5}}{seedance-2.5}：整集连贯性更强，单条质量更弱}
\label{app:seedance}

按自动化评分（\md{seedance-2.5} 没有人工标注），在配对题上，新版本在分镜视频上变差，在集分镜视频与短剧成片上都变好（\cref{fig:seedance}）。
所有必须在时间轴上持续成立的维度都变差了（声画同步 $-0.658$、运动平滑、运镜合理性），
所有关于把镜头接起来的维度都变好了（风格跨镜一致 $+1.143$）。
一个可能的原因是 \md{seedance-2.5} 更字面地遵循提示词，本来就写在提示词里的欠缺也被如实执行
（\cref{fig:seed:case}）；单条从 $15$ 秒拉长到 $30$ 秒，一条镜头里也排进了四次内部切换。

\input{figures/fig_seedance}


\FloatBarrier
\subsection{缺少外部参照时的自动化评分}
\label{app:judgefail}

\input{figures/qual_judgefail}

\cref{fig:qual:judgefail} 是这一失败模式的单题版本：有参照物可核对的维度都判对了，
唯一纯感知的那一维被高估 $3.67$ 分，对应候选指标验证在总体层面所见的失效（\cref{sec:step2}、\cref{tab:axes}）。

